Designing Resource Allocation Tools to Promote Fair Allocation: Do Visualization and Information Framing Matter?

Studies on human decision-making focused on humanitarian aid have found that cognitive biases can hinder the fair allocation of resources. However, few HCI and Information Visualization studies have explored ways to overcome those cognitive biases. This work investigates whether the design of interactive resource allocation tools can help to promote allocation fairness. We specifically study the effect of presentation format (using text or visualization) and a specific framing strategy (showing resources allocated to groups or individuals). In our three crowdsourced experiments, we provided different tool designs to split money between two fictional programs that benefit two distinct communities. Our main finding indicates that individual-framed visualizations and text may be able to curb unfair allocations caused by group-framed designs. This work opens new perspectives that can motivate research on how interactive tools and visualizations can be engineered to combat cognitive biases that lead to inequitable decisions.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by $Author: jpeltier $ $Date: 2007-04-03 16:51:34 -0700 (Tue, 03 Apr 2007) $
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored
by the IEEE Visualization & Graphics Technical Committee (VGTC). This
includes:

Conferences that use the 'conf' document option:
- IEEE Virtual Reality
- IEEE Symposium on 3D User Interfaces
- Symposium on Haptic Interfaces for Virtual Environment and Teleoperator Systems
- IEEE Symposium on Asia Pacific Visualisation
- IEEE Symposium on Interactive Ray Tracing
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Visualization Conference (Posters Only)
- IEEE Information Visualization Conference (Posters Only)
- IEEE Symposium on Volume Graphics

It contains 11 files/directories:

README          - this file
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default conference mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> archives/archive-with-comments-Sep14/00-abstract.tex <==
\begin{abstract}

Humanitarian decisions like charitable donations have been studied in psychology and information visualization. 
Studies have found that cognitive biases such as compassion fade can hinder the fair allocation of humanitarian resources. 
However, few studies have explored how to promote fairer resource allocation.
This work investigates whether the design of interactive resource allocation tools can affect allocation fairness. 
We specifically study the effect of presentation format (using text or visualization) and information framing (showing resources allocated to groups or individuals). 
We ran three crowdsourced experiments where we provided participants with different tool designs to split money between two fictional programs that benefit communities of different sizes. 
Our study did not find conclusive evidence that either presentation format or framing greatly impacts allocation fairness. 
Participants made relatively fair allocations overall, suggesting that with the aid of an interactive allocation tool, people are less prone to compassion fade than has been observed in the past.
%Participants made relatively fair allocations overall, suggesting that with our scenario and allocation tool, people are less prone to compassion fade than has been observed in the past.

% Role of Visualization and Framing in a a resource allocation tool to promote fair allocations

% Visualization and Framing 

% Can Visualization and Information Framing in Resource Allocation Tools Promote Fair Allocations?


% Last version -- 
% Humanitarian decisions like charitable donations have been studied in psychology and information visualization. 
% Studies have found that cognitive biases such as compassion fade can hinder the fair allocation of humanitarian resources. 
% However, few studies have explored how to promote fairer resource allocation. 
% This work investigates the effect of presentation format (using text vs. visualization) and information framing (showing resources allocated to individuals vs. communities) on allocation fairness.
% We ran three crowdsourced experiments where we provided participants with an interactive tool to split money between two fictional programs that benefit communities of different sizes.
% %In four conditions, we presented participants with tools that vary in presentation format and information framing to aid them allocate money.
% Our study did not find conclusive evidence that either presentation format or framing greatly impacts allocation fairness. Participants made relatively fair allocations overall, suggesting that with our scenario and allocation tool, people are less prone to compassion fade than has been observed in past studies.


% Luiz's version -- 151 words
%Humanitarian decisions like charitable donations have been studied in psychology and information visualization. Studies have found that cognitive biases such as compassion fade can hinder a fair allocation of resources. However, few studies have explored how to promote fairer resource allocation. This work investigates the effect of presentation format (text vs. visualization) and information framing (focusing on information about individuals vs. communities) on allocation fairness. We ran three crowdsourced experiments and asked participants to split money between two programs that benefit communities of different sizes. In four conditions, we presented participants with tools that vary in presentation format and information framing to aid them allocate money. Our study did not find conclusive evidence that either presentation format or framing greatly impacts allocation fairness. Participants made relatively fair allocations overall, suggesting that with our scenario and allocation procedure, people are less prone to compassion fade than has been observed in past studies.

% Pierre's version -- 154 words
%Humanitarian decisions like charitable donations have been studied both in psychology and information visualization. However, studies have mostly focused on how to increase donations towards a single charity program, and few have looked at how to promote fair resource allocation. Yet cognitive biases such as compassion fade can hinder fair resource allocation. Through a task involving splitting money between two charities focusing on communities of different sizes, we investigated the effect of presentation format (\textit{text} vs. \textit{visualization}) and information framing on allocation fairness. We used \textit{individual framing}, which emphasizes resources allocated to individuals, and \textit{group framing}, which emphasizes resources allocated to communities. We ran three crowdsourced experiments but did not find conclusive evidence that either presentation format or framing greatly impacts allocation fairness. Participants made relatively fair allocations overall, suggesting that with our scenario and allocation procedure, people are less prone to compassion fade than has been observed in past studies.

%%% Fanny's (?) version -- 189 words 
%Decisions which involve allocating resources such as donating to charitable causes are subject to cognitive biases, including availability bias, compassion fade, or framing effects. Prior studies have focused on mitigating these cognitive biases to promote greater allocation towards a singular cause, but few have investigated how to promote fair distributions, i.e. achieving equitable resource distributions across similar charities. Through a fictional scenario involving allocating resources between two charities serving communities having similar needs but of different sizes, our work investigates the effect of manipulating presentation of the same information regarding resources allocation. We investigate whether individual vs. group framing influences people's decision, i.e. donations contributed towards each individual vs. donations contributed towards each community in both a textual and a visualization presentation. Based on three crowdsourced experiments, we find inconclusive evidence that framing for either text or visualizations has an impact on donation behaviour. Our results show that people make relatively fair distributions in our scenario, suggesting that, provided with an explicit tool that directly presents resource allocation between two charities, people are less prone to compassion fade as previously observed in similar contexts.


%%% ARNAV's draft -- v1
%Decisions which require the allocation of resources such as charitable donations can be difficult to perform due to cognitive biases like framing effects or compassion fade.
%Prior studies have focused on mitigating these cognitive biases to promote greater allocation towards a singular cause but few have investigated how to promote fair distributions such as performing equitable resource distributions across similar charities.
%Our work investigated the addition of numerical information and visualizations, based on two different types of framings, within a decision making interface on making fair distributions. Our framing focused on donations contributed to a group compared to donations contributed towards an individual.
%Based on three crowdsourced experiments, we find inconclusive evidence that the addition of visualizations and changes in framing for either text or visualizations have an impact on donation behaviour. Our measurements show that people make relatively fair distributions, bypassing cognitive biases previously observed in similar contexts.
\end{abstract}



==> archives/archive-with-comments-Sep14/01-introduction.tex <==
\section{Introduction}

People tend to favor humanitarian causes which they feel socially connected to \cite{caviola2021psychology}, leading to isolated communities in need of urgent care with significantly fewer resources.
When a tornado tears down a town in Ohio, charitable Canadian donors may provide an excess of monetary support to help with the rebuilding process while leaving little financial aid to a rural community in Nicaragua devastated from a similar disaster.
In scenarios like these, it is critical that resources are allocated in a \flag{fair} manner between charities, so that different communities which might benefit from different charities can each receive a fair amount of support.

While there are many aspects to be considered when making a allocation, such as assessing its effectiveness for providing aid \cite{gabriel2017effective}, there are also inherent biases to which people can be \flag{privy to, unbeknownst} to them.
Many cognitive biases have been observed \flag{from} prior research in cognitive and social psychology where \flag{affective choices} (like charitable donations) are involved, especially when looking at choices like making a decision which requires the allocation of resources, like time or money.
For example, when presented with numbers which communicate the loss of life, people tend to feel more compassion towards a small number of individuals than a significantly large number \cite{butts2019helping}.
This can mean that people are potentially willing to donate \$100 to 10 people in distress, but only \$110 when there are 100 who need aid, even if they have excess to donate.

Effective donations, like the equitable allocation of resources across similar charities, are preferable. However, they are often not possible.
Due to implicit cognitive biases, a charitable donor might struggle to decide how to split their donations among similar charities or decision makers of government agencies may confuse which charitable programs have excess resources while others have too few.
Different methods of presentation have been tried to alleviate these concerns, however even visualizations which are used to communicate information on charitable programs can often be prone to biases like the framing effect \cite{hullman2011visualization}. 
This can encourage the viewer to associate certain trends or visual effects with a positive or negative connotation, even if none was intended.

Considering the complexities of information presentation, designing tools which help people make fair and equitable resource allocation decisions across multiple groups, such as for charitable donation, is needed. 
Many tools and visualizations currently only focus on encouraging their audience to donate or contribute more towards a specific cause. 
Charity websites may try to convince people to donate more to a specific cause and newspaper articles may try to use photography as means to elicit empathy for the people affected in tragedies \cite{jenni1997explaining}, but few promote unbiased comparisons.
Donation websites such as donorschoose.org or fundraising platforms like gofundme.com allow users to search for similar causes, but comparison across these causes is done by the user with no guided tool, potentially leading to the presence of many biases.

While past works have looked the framing of numerical information in decision making tasks \cite{kahneman1981simulation}, the validity of these designs to promote effective resource distributions, especially for support tools, is unclear.
Currently, research on using visualizations for humanitarian purposes has focused more on how to have people donate more than more effectively \cite{gabriel2017effective}.
Data visualization components like anthropographics \cite{morais2020showing} can also be used to design tools which help bring an emotional connection the data, but does not research the goal of unbiased assessments.
Techniques like framing and nudging have also been studied for computer interfaces \cite{mota2020desiderata, cockburn2020framing} however they do not take into account affective cognitive biases or the use of visualizations into consideration. 

In our work, we fill this gap by investigating how to present textual information and visualizations in a decision making interface such that people are encouraged to make more fair and equitable allocations. 
We further contrast the role of textual framing in influencing how visualizations may be perceived and examine if visualization serves as a reinforcement or mitigation strategy to promote fair and evenly distributed resource allocation across similar causes. 
We accomplish this by presenting different visual and textual framing in a web interface used allocate resources between two charities, across three separate experiments with large population samples (N = 239, 244, 495). 

% We observe that visualization are able to assist when information only surrounding the donation amount 



% \arnav{Audience:} 


% \arnav{Problem Framing:}
% Not much research on resource allocation of pre-existing resources?


%-------

% Charitable causes often do not receive sufficient resources to have their needs met effectively.
% As such, it is critical that all resources given to a cause are allocated in a fair manner.
% % There have been a

% % Remove
% To aid with this, news outlets and journals currently present visualizations which attempt to convey the size or impact of allocations. 
% Some examples include \arnav{Add Examples?}.

% However, there have been few attempts at understanding the utility and benefit that these visualizations have for their observers.
% Understanding the influences that resource allocation visualizations have on users can be significant factor in swaying public opinion and the amount of aid which is given different to programs around the world.

% Not only does this impact government spending but also community donations as the perceived benefits of a donation should align with the amount donated.
% However, perceived benefits are highly subjective for every individual.
% While this may help bring critical aid to some charities, it also means that others which are in need of similar aid are often passed over.

% % What is the topic?
% Information and visualizations about how resources are being allocated can provide people with a means to asses their beliefs on the benefits of their allocation.
% Since this can significantly impact how similar causes receive resources, such information must be presented and communicated in a carefully constructed manner.

% % Background / Examples?
% Prior works have emphasized raising awareness based on factors like importance, urgency, severity of concerning issues, however more broad communication of numbers for such decisions is not well understood [cite]. 
% For example, studies have suggested that when reading numbers which communicate the loss of life, a sense of compassion or empathy is often felt significantly more towards the collective group of people rather than for each of the specific individuals within the group \cite{butts2019helping}. 
% This would mean that people may feel some level of grievance towards the many individuals who have died from a virus like COVID-19, but often do not internalize the disparity between ten or one hundred individuals dying. 

% % Establish research problem
% Psychological studies indicate that having individuals which audiences can relate to emotionally can curb this behaviour [cite], however such approaches do not scale for large and diverse populations.
% For our study, we investigate how numerical framing and the visualization of numerical values affects donors in making judgements about resource allocations.

% % Specify objectives
% By examining the presentation of such design elements, we aim to study how users behave when being presented with summarized information about resource allocations.
% Specifically, we examine if visualization serves as a reinforcement or mitigation strategy to promote fair and evenly distributed resource allocation across similar causes. 
% We also contrast the role of numerical framing in influencing how visualizations may be perceived.

% % Map out paper?
% % In the following sections, we review previous psychological effects which have been observed when presenting information for resource allocation tasks and visual designs which may be used for presentation. 
% % For each experiment, we outline our donation allocation task between two charities and analyse how different design elements influence task responses.
% \arnav{reword}
% In a first experiment, we create two interactive visualizations and differ two numerical strategies to confirm which psychological effects have influences in each design strategy. 
% We find that text framing for numbers produces a statistically significant effect when allocation judgements however different visualizations do not reinforce allocation decisions. Through manual coding of participant responses, we also find participants diverging in their definition of fairness when donating between two charitable programs.

% In a second experiment, we reinforce certain interpretations of fairness by narrowing the scope of the story by better defining fairness. 
% We also narrow our preregistered analysis for different allocation strategies to reflect a simpler categorization, in order to achieve greater statistical power. 
% We discover that participants donate similarly across all conditions once a stricter scope for fairness has been described within the story.

% In a third experiment, we partition our numerical and visualization presentation design in the allocation task with finer detail, testing a larger group (N = 512) to understand the role of a more specific design criteria. 
% We observe that visualization are able to assist when information only surrounding the donation amount 


==> archives/archive-with-comments-Sep14/02-background.tex <==
% Talk about resource allocation 
\section{Related Work}\label{sec:related_work}
In this section we outline prior biases that have been observed to affect decision making behaviour, especially when considering affective, i.e emotional, judgements such as resource allocations.
We further inspect the bias of framing effects and their presence in the presentation of numbers, visuals and interfaces.
Finally, we outline research which has tried to investigate or curb cognitive biases when designing interfaces and visualizations.

\subsection{Cognitive Biases}\label{section:cog_bias}
People may implicitly make biased choices when interpreting information about the availability of resources and making a decision of where they should be allocated.
Sources of bias can come from many areas such as affect.
Since many resource allocation decisions involve a significant affective, i.e emotional, component, such as a charitable donation, we cover past literature which has mapped cognitive processes that can influence a person's actions in decisions regarding resource allocations and other affective scenarios.

Affective decisions can be emotionally laden and unlike deliberative decisions which can take careful information processing, these encourage users to make decisions based on their feelings \cite{dickert2011affective}.
When information is emotionally burdensome however, it can introduce many biases which can cause people to alter their resource allocation behaviour.
The \emph{compassion fade} or \emph{compassion fatigue} effect is a cognitive bias which refers to a decrease in helping or compassionate intent and helping behaviour as the number of people increases \cite{butts2019helping, maier2015compassion, slovic2007affect, bhatia2021more}.
An example of such an effect would be when a donor gives \$300 to a Charity supporting one child but only \$500 to a charity supporting 50 children.
Similarly, the psychophysical numbing or the \emph{psychic numbing} effect occurs when people exhibit diminished sensitivity in valuing lifesaving interventions against a background of increasing numbers of lives at risk \cite{fetherstonhaugh1997insensitivity}.
This effect is similar to compassion fade as it describes a reduction affective emotion, however where compassion fade is for observed external behaviour, psychic numbing is instead for affecting the users internal beliefs and values.

The act of just observing choices to make decision can also induce bias.
The \emph{diversification bias} effect states that people will try to allocate a limited set of resources evenly over the number of possible choices \cite{benartzi2001naive}, i.e donating across multiple different charities regardless of whether some charities need the money more than others.
However other effects can counteract giving evenly. 
For example, the \emph{drop in the bucket} effect refers to when people feel that helping a single or few people may feel like it’s accomplishing nothing \cite{friedrich2010individual}. 
Similarly, the \emph{proportion dominance} effect shows that people favour saving a greater proportion of the population, even though it may mean saving fewer lives \cite{bartels2006proportion}.

\subsection{Framing Effects}\label{section:framing}
Tools which compare resource allocations need both numerical and visualization components to relay information about allocations.
Thus, understanding biases communicated by the different framings presented within these components is critical before trying to understand the interface or design of the tools.

Framing effects are a type of cognitive bias which influence people based on how some type of information is presented.
Framing is used to describe how we communicate information and how that can lend itself to different interpretations \cite{kahneman1981simulation}.
Unlike like more affective cognitive biases which consider the emotional impact for someone, framing effects focus only on impact driven through alternate methods of presenting information.


\subsubsection{Textual Framing}
Textual framing have been well established in existing literature and simply applies the concept of framing towards numerical values integrated in text phrases.
Specially, numerical framing alters the numerical values or creates a different phrase to communicate the same fact.

A foundational example is by Kahnman et al. (1981) \cite{kahneman1981simulation} concerning the loss of human lives which validates that a majority of participants consistently avoid choosing a more risky option when looking a framing to save lives but do the opposite when looking at a framing concerning losses only .
For example, people prefer the text ``200 people will be saved`` compared to ``$\frac{1}{3}$ probability that 600 people will be saved, and $\frac{2}{3}$ probability that no people will be save``. 
However when we frame this as ``400 people will die`` compared to ``there is $\frac{1}{3}$ probability that nobody will die, and  $\frac{2}{3}$ probability that 600 people will die``.

The effect of \emph{entitativity} also shows bias when concerning group belonging in charitable resource allocations. 
When a large number of victims are presented as comprising of an \emph{entitative}, meaning as a single and coherent unit, people will tend to donate more than when they are presented as individuals or statistical numbers \cite{smith2013more}.

\subsubsection{Visual Framing}
Visual framing follows similarly to numerical framing, however instead of text medium as the method of presentation, it is a visual medium such as images or visualizations. 

Many effect have prominently been observed for visual framing.
The \emph{identifiable victim} effect refers to the general principle that people are willing to spend far more money to save the lives of victims which are identifiable, i.e those with individual narratives, than to save statistical victims, i.e those who no story attached to them \cite{jenni1997explaining}. 
While this effect can occur for text framing, it is easy to illicit when showing pictures that an audience can identify with, in place of text.
An example would be showcasing a picture of children in impoverished conditions rather than in a sentence stating that children are in need of aid.

Visualization framing can be considered a subset of visual framing where the visuals are represented as encoded data, and can be useful to communicate things like patterns or scale within the data \cite{franconeri2021science, chevalier2013using}.
The concept of framing visualizations has been studied in many contexts, like in visualization rhetoric which describes framing to influence specific behaviours through visualizations \cite{hullman2011visualization}.
It is important to note however that framing is not the same as rhetoric, as framing does not specifically try to elicit a certain meaning, rather, defines a specific method of presentation which could cause certain meanings to be interpreted.

\subsection{Design for Resource Allocations}\label{section:vis}
Even though there has not been significant research done on developing interfaces and visualizations for resource allocations, there are many design strategies from existing research which can be potentially useful to integrate for such tools.
We looks at past works which attempt to curb cognitive biases, such as those concerning framing, affect, and presentation, in the design of interfaces and visualizations.
We also look at design strategies which can be helpful for presenting and communicating resource allocations as visualizations.

There can be many biases associated with visualizations, for example it has been suggested that people show more interest for visualizations that communicate information may have happened closer to the present \cite{campbell2019feeling}.
Many mitigation strategies have been studied for cognitive biases visualization literature. 
For example, studies show that visualizations which show predictions of future outcomes encourage less optimistic estimates \cite{koval2022you} and being able to remove irrelevant information locally within a visualization to make a comparative decision is able to mitigate some bias \cite{dimara2018mitigating}.

Trying to show specific visuals such as anthropomorphized data graphics, i.e graphics which portray characteristics of humans, has also been tried in order to elicit more prosocial behaviours \cite{boy2017showing}. 
This has been extended in the domain of information visualization with anthropographics \cite{morais2020showing}, however such approaches do not seem to similar prosocial behaviours when conveying human-related statistics \cite{morais2021can}.

More generally, there are visualization design guidelines have been proposed for mitigating cognitive biases \cite{wall2019toward} and eliciting certain beliefs \cite{mahajan2022vibe}, however none have been tested specifically for visualizations in resource allocation tasks and tools.
Frameworks have also been devised to aid in designing visualizations for the proportional representation of resources \cite{chevalier2013using} however they researched in the context of resource allocations or prosocial behaviours specifically.

Direct design of resource allocation tasks such as charitable donations have also been studied. Nudging, where incremental hints are made to favour certain outcomes, has been a method used in interface design to encourage more equitable donations across many different charities as well \cite{mota2020desiderata}.


==> archives/archive-with-comments-Sep14/03-vis-design.tex <==
\section{A Tool for Resource Allocation: Design Considerations}\label{section:framing_res_alloc}

%\begin{figure*}
%        \centering
%        \includegraphics[width=0.45\textwidth]{pictures/num_framing2.png}
%        \caption[]
%        {{Design of the numerical framing shown for all experiments.}}    
%        \label{fig:numerical_framing}
%\end{figure*}

%\begin{figure*}
%        \centering
%        \includegraphics[width=0.45\textwidth]{pictures/exp_framing2.png}
%        \caption[]
%        {{Design of the Anthropographics and Resource Visualization framing shown for Experiments 1-3.}}    
%        \label{fig:exp_framing}
%\end{figure*}


%\begin{figure*}
%        \centering
%        \includegraphics[width=0.8\textwidth]{figures/placeholder-figure.png}
%        \caption[]
%        {{PLACEHOLDER}}    
%        \label{fig:xx}
%\end{figure*}

Imagine that you decide to contribute to humanitarian causes around the world -- how should you split your money if you had two causes to aid? Or think about how big organizations like the United Nations should allocate their funds between the different programs they support. Those are examples of the \textbf{resource allocation problem}. This problem happens when two or more groups should be benefited by the allocation of resources. The question is: how to make effective or fair allocations based on the information that the decision-maker has available?

The problem is complex because, in real-world scenarios, the groups can have completely different characteristics. If we take the example of the two tornado disasters from the introduction, we would have to compare an event that happened in Ohio with another that occurred in a much smaller region in Nicaragua, which probably received less media coverage. All of those factors can play a role in how people make judgements to allocate money. If people choose just based on their own experience or intuition, they might be influenced by cognitive biases and their attitudes. On the other hand, if the donors decide to allocate resources based on data but without a proper tool, they can be overwhelmed by the amount of information.

This paper is a first attempt to explore the design of resource allocation tools to promote fair allocations. We consider resources to be \textit{fairly allocated} when each beneficiary receives the same amount of resources as any other beneficiary, irrespective of the group they belong to. For the sake of simplicity and reproducibility, this research focuses on a task in which all individuals from two groups have comparable needs and contexts, with only the group sizes changing. This way, we make sure that the same amount of resources would benefit different individuals equally. This decision helps breaking the resource allocation problem down into a simpler problem and controls for confounding factors in the experiments we conducted. Possible limitations for this approach are addressed in the discussion section.

In this work, we are particularly interested in the effect of two design dimensions on resource allocation. \textbf{Presentation format} corresponds to how information is represented to the viewer. For instance, we can use \textit{text} to describe the resource split across groups, or a \textit{visualization} for quick visual assessment and comparison. There is also \textbf{information framing}, which is how the message is conveyed to the user. For example, the message could have a \textit{group} framing, which would focus on describing the amount donated to each group, or it could have an \textit{individual} framing, where the message would be focused on how much would be donated to each individual in the groups. We examined how presentation format and information framing affect resource allocation by designing and testing interactive tools that vary in terms of those two dimensions.

In the following sections, we describe in more detail examples of designs that combine different presentation formats and information framings. Lastly, we introduce the interactive tools used in our experiments.

%Imagine you wish to donate to a humanitarian cause, for which different charitable programs provide support for --- program Alpha, which provides aid to a small group of people, and program Zefa, which provides aid to a larger group. To help achieve a \textit{fair allocation} of the available resources to donate, we propose to design an interactive tool that allows donors to directly assess how different splits of resources benefit the respective communities.

%In our research, we consider resources to be \textit{fairly allocated} when each individual receives the same amount of resources as any other individual, irrespective of the program. Note that for simplicity, we assume that all individuals have comparable needs and contexts, i.e. that the same amount of resources would benefit different individuals equally.

%Our proposed tool aims to help people allocate money for a donation across two charitable programs in a fair manner. To make judgement about how resources are allocated across, our tool communicates relevant information about each of the charitable programs, i.e. the name of the program and its size, and the amount allocated to each program. The latter is dynamically updated as the donor adjusts their allocation decision. We discuss how such tool can vary in its design, regarding \textit{how} this information is presented to the donor.

%While saying \textit{``I give \$150 to program A (which has 3 people) and \$200 to Zefa (which has 8 people)''} is technically the same as saying \textit{``I give \$50 to individuals in program Alpha and \$25 to individuals in program Zefa''}, the difference in \textbf{framing} can influence how people process the information. In the former, the focus is on the amount provided to each community, which can obfuscate assessment of how much each individual will receive. On the contrary, the second framing makes that information directly explicit. 

% Further, different \textbf{presentation formats} can be used to convey this information. For instance, we can use text to describe the resource split across the programs, but we can also use a visual representation conveying the quantities we are dealing with, for quick visual assessment and comparison.

%Our work is interested in studying whether varying the design of such tool, regarding the presentation format and framing, affects resource allocation. In the following, we discuss \flag{xxx}, organized by presentation format.


\subsection{Textual Information}\label{sec:text}

One of the most basic components in charitable messages is textual information. Charitable ads are usually composed of a textual description of a problem accompanied by other presentation formats such as a picture or a data visualization. The way the text is framed can affect people's judgements or decisions~\cite{chang2009framing}. In this work, we explore two ways of framing the textual information: focusing on the \textit{group} or on \textit{individuals}.

%How the resources are split between different programs can be expressed by directly utilizing text, i.e. words and numbers. To facilitate quick comparison between the benefiting charities, we opt for a concise form to convey the size of the community, i.e. \textit{``Number of beneficiaries: 3 people"}, the amount that community is currently allocated, \textit{``Current donation: \$800"}, and the amount each individual within the community receives, i.e. \textit{``\$206.7 per person''}. 

When \textbf{textual information} is \textbf{framed by group}, the message is expressed as a total donation to each group (e.g., \textit{"give \$1,000 to aid the victims of Ohio's hurricane and \$300 to help victims of Nicaragua's disaster"}). This framing allows the viewer to think holistically about the allocation given to the respective groups, rather than considering individual beneficiaries. 
%We believe this framing could be prone to compassion fade \flag{[REF]}  or \flag{[psychic numbing]} since groups with large numbers may overwhelm the donor, who may in turn believe that they are donating an irrelevant amount to communities of larger size \cite{vastfjall2014compassion}.
This framing can induce the effect of entitativity \cite{smith2013more} as it can encourage the donor to associate the group of people in each program to singular group units rather than see these communities as a group of individuals. Group framing can also result in the naive diversification bias~\cite{benartzi2001naive}, when people prefer to allocate limited resources evenly across options, even when the options (or groups) have different characteristics.

When \textbf{textual information} is \textbf{framed by individuals}, the message is expressed in terms of the amount received per person (e.g., \textit{"give \$15 to each victim of Ohio's hurricane and \$12 to each victim of Nicaragua's disaster"}). This framing allows the viewer to reason in terms of what individuals in the respective communities each receive, rather than what the group as whole receives. This framing can possibly help alleviate the effect of compassion fade \cite{vastfjall2014compassion}, because breaking down large numbers become more palatable when expressed as what that means for individuals. It could also possibly help alleviate the entivativity effect and the naive diversification bias, since individuality is directly expressed.


\subsection{Visual Information}
\label{sec:visualization}

We can also display the resource allocation information using a data visualization. In our work, we opt for using an iconic representation~\cite{boy2017showing} of people (i.e., icons of a human), and resources (i.e., coins). Like for Isotypes~\cite{neurath1974isotype}, the number of icons encodes the respective quantities, using partial rendering of icons when necessary. See an example in ~\autoref{fig:interface}.

We chose an iconic representation to represent individuals specifically as the true scale of the different communities may be easier to grasp through visual aggregation of icons, than by interpreting numbers in textual form. %Further, representing ``people behind the numbers" as so done in anthropographic visualization \flag{[REF]}, could result in increased empathy towards the people in need of aid. These together can play a role in mitigating compassion fade.
As for the text presentation format, we can play with different organization of icons representing quantities to vary the information framing. We dicuss these below.

\textbf{Visual information} can be \textbf{framed by group} by using Gestalt psychology~\cite{kohler1967gestalt} to create a perception of unity for each group. Icons representing people that belong to specific groups can be located together spatially so that they are visually perceived as a unit, per the Gestalt law of proximity. Similarly, the icons representing resources could be grouped together, so as to be associated perceptually and interpreted as an overall amount of resources allocated to the group. We opt for spatial grouping in this work (see an example in \autoref{fig:exp_1_conditions}-c), but other perceptual groupings could be considered in future designs of a resource allocation tool.

%For each group of icons occupying a spatial partition of the display, different spatial organization within these partitions can be considered, each of which having pros and cons regarding perceptual properties. For instance, a grid layout can outperform a more organic layout with respect to counting how many items are represented and comparing between two distributions, but may feel too organized when it comes to representing communities of people. A compact layout can give a stronger sense of cardinality compared to a sparse layout. In our work, we set a constraint on this choice, so as to not create too much of a confound between different visualization framings, and opted for icons representing idividuals to follow a grid layout, as it better supports individual framing, as described below.


\textbf{Visual information} can be \textbf{framed by individuals} using the same Gestalt principles of perceptual grouping, combining visual representations that correspond to each beneficiary. An individual framing can be created by placing the exact amount of resources allocated to each individual, besides each individual (see an example in \autoref{fig:exp_1_conditions}-d). This way, the donor can easily perceive how much splitting one group's allocation across individuals results in, for each individual within the group.% Comparing between individuals' allocation between different programs is also facilitated, as one can directly compare the difference per individual.



\begin{figure*}[th]
        \centering
        \includegraphics[width=0.6\textwidth]{figures/Interface.pdf}
        \caption[]
        {Screenshot of our instance of an interactive resource allocation tool featuring two charitable programs, utilized in Experiment 1 of our study. With the help of the legend (a), a donor can directly assess the result of resource allocation presented in the information display (b). Here both text and visualization representations are displayed, each presenting allocations with an individual framing. The donor can dynamically adjust how the resources are split between the two programs, using the slider (c), which automatically updates the information presented in the information display.  }    
        \label{fig:interface}
\end{figure*}


\subsection{Putting it all together: An interactive tool for resource allocation}
\label{sec:tool}

% To help a donor form a judgement about whether resources are allocated fairly across, we propose for a resource allocation tool to communicate relevant information about each of the charitable programs, i.e. the name of the program and its size, and the amount allocated to each program. The latter information should be dynamically updated as the donor adjusts their allocation decision. We discuss how such tool can vary in its design, regarding \textit{how} this information is presented to the donor.

We created a resource allocation tool that combined different presentation formats and framings. \autoref{fig:interface} shows a screenshot of the interface we used in our study, for one of the conditions in Experiment 1. The tool is composed of three parts: (\texttt{a}) a legend, which informs the number of people and resources encoded by each mark in the visualization; (\texttt{b}) a display, showing textual and/or visual information about the groups and corresponding resources to be allocated; and (\texttt{c}) a slider, which allows the user to change the amount of resources dedicated to each group. Since we only consider 2-group allocations in this paper, the display (component \texttt{b}) is divided in two parts; one for each program/group. The information shown in the display dynamically changes as the user moves the slider to the left (to benefit group Alpha) or to the right (to benefit group Zefa). That template was used for all of our experiments.

To study how the two dimensions affect resource allocation, we manipulated the tool design in terms of presentation format and information framing. We tested designs composed of only text, visualization (the legend is only shown in conditions where the visualization is present), or both. Also text and visualization had group or individual framings. In the example shown in \autoref{fig:interface}, the display encompasses both textual and visual information, with individual framings for both presentation formats. The text follows an individual framing because it contains the exact amount to be donated for each individual (in blue). The visualization also follows an individual framing because the coins encoding the values allocated to each beneficiary are aligned with the icons representing individuals. As both text and visualization have the same framing, we consider that the tool has a \textbf{congruent framing}. Conversely, when the text and visualization have opposite framings, the tool has an \textbf{incongruent framing}. There are many other aspects to the design of a resource allocation tool that could be considered, which we discuss more in depth in the discussion section. 


%% TALK ABOUT GROUPING IN EACH FRAMING

%While information about the number of individuals in a group is already given in the numerical representation, effects like compassion fade may cause individuals to devalue how much to give based on observing a number.
%Thus, we presumed that adding an marks for the people being supported in the visualization may help emphasize the proper scale of a program and reduce compassion fade.
%Note that the athropograpic glyphs are always centered and spaced evenly and favoured to be at bottom of the tool for experiments 1 and 2. 
%In the group framing condition of experiment 3, we stack the rows of marks for individuals on top of each other, without any other marks in between, as we hoped to exaggerate the effect of \emph{entitativity} which was already present in the numerical group framing.



%    Similarly to the numerical group framing, we believe this framing allows users to think holistically about the resource being allocated to group rather than towards an individual.
%\flag{To encourage users to think of coin being attributed to the group rather than to a specific individual, the coins were also scattered according to poisson-disc sampling in Experiments 1 and 2. We presumed if the coins were not scattered, the user would be able to map the number of coins to an individual easily, negating the motivation behind the framing. However, due to an increase in the number of marks representing a coin in experiment 3 and our qualitative analysis, we opted to remove the scattering aspect as it had minimal impact on how users perceived the design.} \fanny{TODO: add this in the respective sections.}
%    The \emph{visualization person framing}, where the resource allocation visualization shows the amount that each group will receive with glyphs for each resource arranged such that they are alongside each anthropographic. For example, if we were to give \$100 for a group of 10 people, we have 10 group of 10 coins grouped on top of each of the 10 people in the group.
%    Similarly to the numerical person framing, we believe this framing allowed users to think about the resource being allocated to each individual rather than towards the collective group.}
    

\endinput









%%%%%%%%%%%%%%%%%% PREVIOUS VERSION %%%%%%%%%%%



% For our study, we built a user interface to help participants allocate money for a donation across two charitable programs.
% Specifically, we draw a comparison between a program which provides aid to a small group of people, called program Alpha, and a program which provides aid to a larger group, called program Zefa.
% Our interface communicates information about the amount allocated for each charity through two representations, a numerical representation and a visualization representation.
% We look at two different ways of framing each representation to assess the different cognitive biases people may have when interpreting information and making a decision using our interface.

% We do this by contrasting how well the addition of a specific representation or specific framing is able to support the user in allocating resources equally for all individuals in both program Alpha and Zefa, irrespective of group belonging.
% In our research, we call this donating in a \textbf{fair} manner.
% For example, if program Alpha has 3 people and program Zefa as 12 people, allocating \$3000 in a \textbf{fair} manner in our study would be giving \$200 to all individuals, mean \$600 to program Alpha and \$2400 to program Zefa.

% The different framings for our numerical representation is shown in Fig. \ref{fig:numerical_framing} and the framing for the visualization representation is shown in Fig. \ref{fig:exp_framing}.
% In the following sections we explain the role which each of the representations play in influencing users to make fair donations.
% We also identify any potential cognitive biases which may be associated with specific types of framings.

% \subsection{Numerical Representation}
% The numerical representation always shows the name of the group for whom the information is displayed.
% We display up to two additional pieces of numerical information in this representation, each with a different type of framing. The breakdown of the different framings used in our three experiments are shown in Figure \ref{fig:numerical_framing}.

% We classify the two framings as follows:
% \begin{itemize}
%     \item The \emph{numerical group framing}, where the text shows the number of people associated with the group and current total allocation given to the group, i.e 10 people in Group A and \$1000 for Group A.
%     This framing allows users to think holistically about the allocation given to the group rather than to specific individuals.
%     Framing numerical values like these could be prone to \emph{compassion fade}  or \emph{psychic numbing} since large numbers may overwhelm the user to believe that they are donating an irrelevant amount towards the larger group \cite{vastfjall2014compassion}.
%     This framing can induce the effect of \emph{entitativity} as it can encourage the donor to associate the people in each group as singular units rather than as individuals.
%     \item The \emph{numerical person framing}, where the the text shows the amount received per person, which is the allocation amount divided by the number of beneficiaries, i.e \$10 per person Group A.
%     The addition of it allowed users to think in terms of what each person would receive rather than the group as a whole would receive.
%     This can help remove the entivativity effect \cite{smith2013more}, and allows users to compare charities along equal comparisons.
% \end{itemize}

% \subsection{Visualization Representation}
% The visualization representation encodes the data presented in the numerical representation into a visualization, using appropriate marks corresponding to the appropriate data.
% The visuals for this component are shown in Figure \ref{fig:exp_framing}. 
% Two core concepts are represented within all visualizations, the number of people receiving the allocation and the amount of resources being allocated for a group, in our experiments this is the amount of money given to the program.

% \subsubsection{Representing People}
% We represent the number of people being provided aid in a program with human silhouette shaped marks colored in gray for Experiment 1 and 2; and white for experiment 3.
% The change in color acted as a better contrast for accessibility in Experiment 3.

% While information about the number of individuals in a group is already given in the numerical representation, effects like compassion fade may cause individuals to devalue how much to give based on observing a number.
% Thus, we presumed that adding an marks for the people being supported in the visualization may help emphasize the proper scale of a program and reduce compassion fade.
% Note that the athropograpic glyphs are always centered and spaced evenly and favoured to be at bottom of the tool for experiments 1 and 2. 
% In the group framing condition of experiment 3, we stack the rows of marks for individuals on top of each other, without any other marks in between, as we hoped to exaggerate the effect of \emph{entitativity} which was already present in the numerical group framing.

% \subsubsection{Representing Resources}
% The amount of money given to the program is represented with an mark of a stack of coins for Experiments 1 and 2; or a mark using a yellow circle, acting as an abstract representation for a coin, for Experiment 3.

% Two separate framings alter how we present the marks for the resource allocation as follows:
% \begin{itemize}
%     \item The \emph{visualization group framing}, where the resource allocation visualization shows the amount that each group will receive with the marks for each resource arranged such that they are separated from the mark for the individuals receiving the aid. For example, if we were to give \$100 for a group of 10 people, we have 100 coins grouped on one side and 10 marks people group on another side.
%     Similarly to the numerical group framing, we believe this framing allows users to think holistically about the resource being allocated to group rather than towards an individual.
%     To encourage users to think of coin being attributed to the group rather than to a specific individual, the coins were also scattered according to poisson-disc sampling in Experiments 1 and 2. We presumed if the coins were not scattered, the user would be able to map the number of coins to an individual easily, negating the motivation behind the framing. However, due to an increase in the number of marks representing a coin in experiment 3 and our qualitative analysis, we opted to remove the scattering aspect as it had minimal impact on how users precived the design. 
    
%     \item The \emph{visualization person framing}, where the resource allocation visualization shows the amount that each group will receive with glyphs for each resource arranged such that they are alongside each anthropographic. For example, if we were to give \$100 for a group of 10 people, we have 10 group of 10 coins grouped on top of each of the 10 people in the group.
%     Similarly to the numerical person framing, we believe this framing allowed users to think about the resource being allocated to each individual rather than towards the collective group.
    
% \end{itemize}

% \section{Study Design}
% In this study, we investigate the role of visual framing when pertaining to the design of visualizations which convey resource allocations.
% To accomplish this, we conduct three experiments which ask participants to make a charitable donation between two charities after reading a story about two competing programs.
% In order to donate, each participant must use an interface with  certain text or an additional visualization, adhering to a certain framing criteria as discussed in the previous section.






==> archives/archive-with-comments-Sep14/04-studysetup.tex <==

\section{Experimental Design: Overview}
\label{sec:expe-design}

We conducted a series of three experiments to gain a better understanding of how people approach the resource allocation problem in a fictional scenario. Each experiment builds on findings and lessons learned from the previous experiment(s). In this section, we describe the general context for our study, and overall procedure common to the experiments. Elements specifics to a particular experiment are discussed in the corresponding sections. All experimental materials, procedures, and pre-planned analyses were pre-registrered for each of our experiments independently\footnote{All pre-registration materials can be found at \url{https://osf.io/xqser?view_only=1049a79a474a4310958571269aa5e248} (Experiment 1), \url{https://osf.io/7ebsm/?view_only=4ff3f6ae865f444282ecd95de4a302b0} (Experiment 2) and \url{https://osf.io/egv85/?view_only=e702e7de07114e18bebd175aa0d8b43b} (Experiment 3)}.

\subsection{Task}
\label{sec:task}
We created a fictional scenario for the resource allocation task. Participants were provided with a brief about a charitable organization which is helping setting two separate programs for impoverished children. The scenario brief specifies the charity's mission is to aid children around the world, and emphasizes that the money which the participant is asked to allocate will be of significant value to accomplish this goal. The participant was informed that:
\begin{quote}
\textit{``Your task is help the organization decide how to distribute money between two of their programs.''} 
\end{quote}

\noindent The two programs, Alpha and Zefa, differ in size:  Alpha aids less children than Zefa does (specific sizes are reported in the respective sections). The brief also specified how the money will be utilized (i.e., \textit{`` the money will go toward food, clothes, and education''}). Further, the brief includes little information about the individuals in each program, as we wanted to measure the presentation of summarized information rather than the presentation of identifiable victims.

%To minimize opportunities for participants to speculate on other factors that might influence their decision, the brief also provides a description of how the money will be utilized (i.e., \textit{`` the money will go toward food, clothes, and education''}), and that the resources that the participant is tasked to allocate is the sole resource for the programs (i.e., \textit{``[Children] will not benefit from any other donation than yours.''}). Further, the brief includes little information about the individuals in each program, as we wanted to measure the presentation of summarized information rather than the presentation of identifiable victims.

%Participants were told that they have a given amount of money to allocate in full between the two charity programs:
%\begin{quote}
%    \textit{``All the money you donate to a program will be split evenly between the children in the program.''}
%\end{quote}


Our scenario was inspired from the scenarios that are found in psychological studies investigating the effects of the victim size on resource allocation~\cite{garinther2022victim}. In our experiments, we  chose to keep population sizes for each program relatively small, i.e not in the thousands or millions, as similar studies had shown that compassion fade is based on the proportional difference between populations \cite{maier2015compassion}. This means the effect observed in our experiments would theoretically hold if population sizes were tens or hundreds times larger. Since a smaller population number can be easier for participants to reason about, we chose population sizes of small magnitudes as found in similar studies \cite{garinther2022victim}.


\subsection{Procedure}
\label{sec:procedure}
We deployed our experiment online. Upon sign up, eligible participants were directed to a self-hosted website where they were first asked to give consent. Participants who consented were presented with the scenario and task (see \S \ref{sec:task}). When proceeding to the next screen, they were presented with the interactive tool to make their allocation (see \S \ref{sec:tool}). Participants were not instructed anything more than allocating resources between the two programs as they saw fit. No indication of performance goals was provided, i.e. participants were not hinted at what would be a reasonable or desirable split of resources, neither were they given time or speed constraints.

After submitting their choice for resource allocation, participants were asked to explain the rationale for their choice briefly, in an open text box. We did not inform participants that they were going to be asked to justify their decision until after they decided how to split the resources between the programs, and participants were not allowed to return to the previous screen to change their allocation. We did so to minimize potential social desirability bias~\cite{fisher1993social} which may arise when one feels they are being held accountable for their decision (which is also why we opted against a donation intention question for our task). We also asked participants include the confidence in their choice, on a five-point Likert scale, from ``not at all confident'' to ``very confident''. 

Finally, participants were posed a multiple-choice question about the purpose of the charity, which we used as an attention check to exclude potentially inattentive participants or bots, whose responses would introduce noise.

\subsection{Measurements.}
\label{sec:measurements}
Our primary measurement is obtained from the slider (\autoref{fig:interface}-c) which  records how the full amount of available resource was split between the two programs. We 
developed metrics to gauge the extent to which allocations were \textbf{fair or unfair}, which we describe in each Experiment's section. We also characterized what different allocation values mean in terms of \textbf{allocation strategy} employed, which we describe below.

Consider the example where splitting a \$3,000 donation such that Zefa is allocated \$2,400 results in each individual receiving the exact same amount in both programs (these correspond to values used in Experiments 1 \& 2). There are two main allocation strategies which we can measure for, considering values donated to Zefa in such scenario:
\begin{itemize}
    \item The \emph{\textbf{fair allocation}} $\in \{ 2400 \}$ strategy which treats all children equally, i.e. money is allocated in such a way that individual people in the two programs get the same amount of money. Note that this allocation favors the larger program (Zefa), in that more money (\$2,400) is allocated to it compared to Alpha (\$600). But this strategy treats individual people equally, which can be conceptualized as the allocation strategy that is fair towards individuals. 
    \item The \emph{\textbf{unfair allocation}} $\in [0,3000] - \{2400\}$ strategy encompasses any other allocation, where children in different programs are aided a different amount of resources.
\end{itemize}

We further break down the \emph{\textbf{unfair allocation}} strategy into four subcategories as follows:

\begin{itemize}
\item The \emph{\textbf{minority-skewed allocation}} $\in$ $[0, 1500)$ strategy favors the program with less people, indicating that the participant has donated between \$0 and under \$1,500 to program Zefa. 
Thus, more money is allocated to the program with the smaller number of children. 
The allocation favors both the smaller program (Alpha) and the individual people in this program.

\item The \emph{\textbf{naive allocation}} $\in \{1500\}$ strategy treats the programs and their causes equally, indicating that the participant has donated exactly \$1,500 to program Zefa. 
Thus, the same amount of money is allocated to the two charity programs.
The allocation treats charity programs equally but favors individual people in the smaller program (Alpha). 
This response is indicative of a diversification bias \cite{benartzi2001naive}. 

\item The \emph{\textbf{mixed allocation}} $\in (1500, 2400)$ strategy balances causes and beneficiaries, indicating that the participant has donated at least over \$1,500 but under \$2,400 to program Zefa. 
Thus, more money is allocated to the program with the larger number of children (Zefa), but individual people from the smaller program (Alpha) still get more money. 
This type of response is indicative of a compassion fade effect \cite{butts2019helping}.

\item The \emph{\textbf{majority-skewed allocation}} $\in (2400,3000]$ strategy favors the program with more children, indicating that the participant has donated at least over \$2,400 and up to the maximum amount, \$3,000 to program Zefa. 
Thus, more money is allocated to individual people in the charity program with the larger number of children (Zefa). 
The allocation favors both the larger program and the individual people in this program.

\end{itemize}



%We define giving a \textbf{fair} allocation as giving equally across all individuals, irrespective of group belonging.
%For example, in experiments 1 and 2 we ask users to allocate \$3000 between programs \emph{Alpha} (3 children) and \emph{Zefa} (12 children).
%In this case, a fair allocation would mean giving \$600 to Alpha and \$2400 to Zefa, meaning \$200 per individual, irregardless of the program that belong to.

%There are many metrics which we can use to measure if a user has achieved perfect fairness within their allocation between programs. 
%The following outlines and contrast different metrics with continuous domains which can be used to measure the closeness to a fair distribution that the user has achieved.


\subsection{Analyses.}
\label{sec:analyses}

We performed inferential statistics and draw our inferences from graphically-reported point and interval estimates \cite{cumming2005inference}. All our effects are estimated by using the percentile method of obtain 95\% bootstrapped confidence intervals (CIs). We also do not adjust for multiplicity \cite{bender2001adjusting, li2017introduction}.

We also performed a qualitative analysis of the content of the free-text responses to the question asking participants to justify their choice. Methods used are described for each Experiment.


\subsection{Recruitment, Inclusion \& Exclusion Criteria}
Participants were recruited through the Prolific crowdsourcing platform, which was chosen for its larger set of positive actors compared to other similar platforms \cite{gupta2021experimenters}. In a pre-screening process, participants were required to speak English fluently, to have a 99\% approval rate on the Prolific platform, and to have not participated in any of our pilots in this project to be eligible. We also recruited only from majority English speaking countries, namely, the UK, USA, and Canada. We excluded data from participants who did not complete the study, or failed at answering correctly the attention test (see \S \ref{sec:procedure}).

\endinput


% \arnav{talk about slider and stuff}

\subsection{Procedure}
We asked all participants to navigate through a series of pages by clicking a button labeled "next" at the bottom of their screen. 
They were not allowed revisit each page through any means.

Before starting the study, participants were shown a brief description of the study and then a detailed overview alongside the details of consent on pages 1 and 2.
No insights or explanations about the tool design were related to the user on either screen.

Upon consent, participants were shown a story (see \S \ref{ssection:story}) describing the context behind the charitable programs. 
At the end of the story, participants are told that they have \$3000 (USD) to allocate between the two charity programs.
Participants were shown the tool to allocate between program Alpha and program Zefa.

Upon making their allocation and proceeding forward, participants were given three questions. 
Questions 1 asked participants to explain their choice choice, questions 2 asked how confident the participant was for their choice, and question 3 acted as an attention check where the participant had to pick the purpose of the charity from six choices. 
All questions were required to be answered finishing the experiment.

Upon completion, we upload the results to our cloud-hosted database and displayed a link to return to the experimental platform (Prolific) which indicated that they had completed the study.

The values uploaded to our cloud database were: their starting timestamp, their finishing timestamp, three identifier parameters given by prolific, the type of framing they were given, the presentation format they were given, the amount the allocated to program Zefa, and their responses to all three questions.





\subsection{Story}\label{ssection:story}

Participants are first introduced to a story about a charitable organization which is helping set up two unique programs for children.
% We specify the charity's mission to aid children around the world and emphasize that cost effectiveness is of significant value to accomplish this goal.
Two programs are then introduced which both provide money and similar materials to support children in both programs. 
%Both the program description and story contained little information about individuals as we wanted to measure the presentation of summarized information rather than the presentation of identifiable victims.(IVE)


% ref: https://docs.google.com/document/d/1nOcE_dud_lFtwAf4pA13krIHC7ThE6SZPE9IlYqdr-g/edit
%We base our story similarly to ones present in previous psychological studies which try to investigate the effects of the victim size for resource allocation scenarios \cite{garinther2022victim}.
We specify the charity's mission to aid children around the world and emphasize that cost effectiveness is of significant value to accomplish this goal.
The Two programs are then introduced which both provide money and similar materials to support children in both programs. 
We label Program \emph{Zefa} as a program which support a larger subset of children while program \emph{Alpha} supports a small subset.
In experiments 1 and 2 we set \emph{Alpha} to aid 3 children and \emph{Zepha} to aid 12. While in experiment 3, we set \emph{Zepha} to have 120 children.
Both the program description and story contained little information about individuals in each program as we wanted to measure the presentation of summarized information rather than the presentation of identifiable victims.

We explicitly choose to keep population sizes for each program relatively small, i.e not in the thousands or millions, as similar studies had shown that compassion fade is be based on the proportional difference between populations \cite{maier2015compassion}. 
This means the effect would apply similarly if both population sizes were 10x larger, so for example, compassion fade would apply similarly if we had a population comparison of 30 vs 120 than compared to our 3 vs 12.
Since a smaller population number can be easier for participants to reason about, we choose the smallest population comparison in similar literature \cite{garinther2022victim}.

At the end of the story, participants are told that they have \$3000 (USD) to allocate between the two charity programs. This allocation amount was chosen as it provides a realistic amount which charities may use when dealing with budget restrictions for different causes [cite].

We ask three additional questions regarding their choice afterwards. The first question asked participants to briefly explain their choice. 
The second was the confidence in their choice, on a five-point Likert scale, from "not at all confident" to "very confident". 
The third question was presented on a separate page and acted as an attention check, asking about the purpose of the charity they read about.

% A "next" button is presented at the bottom which takes them to a different screen where information about their allocation to each program is presented for the donation task, as per one of the four condition in Figure \ref{fig:exp_1_design}.

\subsection{Resource Allocation Interface}
\begin{figure*}[t]
        \centering
        \includegraphics[width=0.90\textwidth]{pictures/exp_preview.png}
        \caption[]
        {{A example of the allocation screen for Experiment 3 with the (noNum, personVis) condition.}}    
        \label{fig:numerical_framing}
\end{figure*}



\subsection{Measuring Fairness}\label{ssection:measure_fair}
\begin{figure}
    \centering
    \includegraphics[width=0.47\textwidth]{pictures/slider4.png}
    \caption[]
    {{\small Allocation values for different breakpoints on the tool's slider.
    Note: The distance between values may not be completely at scale.}}    
    \label{fig:slider}
\end{figure}

We define giving a \textbf{fair} allocation as giving equally across all individuals, irrespective of group belonging.
For example, in experiments 1 and 2 we ask users to allocate \$3000 between programs \emph{Alpha} (3 children) and \emph{Zefa} (12 children).
In this case, a fair allocation would mean giving \$600 to Alpha and \$2400 to Zefa, meaning \$200 per individual, irregardless of the program that belong to.

There are many metrics which we can use to measure if a user has achieved perfect fairness within their allocation between programs. 
The following outlines and contrast different metrics with continuous domains which can be used to measure the closeness to a fair distribution that the user has achieved.

The \textbf{Large Program Allocation} consists of the raw value the user has allocated towards the largest program. Since, we only have two programs in our study, a fair allocation would mean \$2400 being allocated to \emph{Zefa}, the program with a larger population.

This measure is also less likely to suffer from social desirability bias than donation intention questions (e.g., how much participants report they would be willing to donate to a single charity) \cite{fisher1993social}.

The \textbf{Unfairness Distance} measure is the distance to a fair allocation. 
For the sake of clarity we assign this measure the unit \texttt{UFD} standing for (U)n(F)airness (D)istance.

Having 0 \texttt{UFD} would mean a fair allocation has been made, i.e  \$2400 allocated to Zefa.
However, the further from zero, the unfairer the allocation it. For example, a value of 600 \texttt{UFD} could mean \$3000 or \$1800 has been allocated to Zefa, both of which are a distance of 600 away from a perfectly fair allocation which is \$2400.

We note that \texttt{UFD} can be equivalently compared to popular metrics such as the GINI coefficient, which could be seen as a normalized form our distance metric. 
However we wanted to use a metric which preserves our exact allocation value for both programs as specific breakpoints might derive additional meaning in the context of our allocation strategies. 

\subsection{Allocation Strategies}\label{sssec:alloc_s}
In this section we cover possible allocation strategies. We provide example sets using the Large Program Allocation metric for the first two experiments (i.e donating up to \$3000 to program Zefa).

There are two main allocation strategies which we can measure for:
\begin{itemize}
    \item The \emph{\textbf{fair allocation}} $\in \{ 2400 \}$ strategy which treats beneficiaries equally, indicating that the participant has donated exactly \$2400. 
    Thus, money is allocated in such a way that individual people in the two programs get the same amount of money. 
    The allocation favors the larger program (Zefa) but treats individual people equally. 
    This can be conceptualized as the allocation strategy that is fair towards individuals. 
    \item The \emph{\textbf{unfair allocation}} $\in [0,3000] - \{2400\}$ \arnav{rewrite}
    strategy where more money is allocated to individual people in the charity program with the larger number of beneficiaries (Zefa). 
    The allocation favors both the larger program and the individual people in this program.
\end{itemize}

We break down the \emph{\textbf{unfair allocation}} strategy further into four other subcategories as follows:
% \arnav{explain why we break down to more finite?}
\begin{itemize}
\item The \emph{\textbf{minority-skewed allocation}} $\in$ $[0, 1500)$ strategy favors the cause with less beneficiaries, indicating that the participant has donated between \$0 and under \$1500 to program Zefa. 
Thus, more money is allocated to the charity program with the smaller number of beneficiaries. 
The allocation favors both the smaller program and the individual people in this program, program Alpha.

\item The \emph{\textbf{naive allocation}} $\in \{1500\}$ strategy treats the programs and their causes equally, indicating that the participant has donated exactly \$1500 to program Zefa. 
Thus, the same amount of money is allocated to the two charity programs. 
The allocation treats charity programs equally but favors individual people in the smaller program (Alpha). 
This response is indicative of a diversification bias \cite{benartzi2001naive}. 

\item The \emph{\textbf{mixed allocation}} $\in (1500, 2400)$ strategy balances causes and beneficiaries, indicating that the participant has donated at least over \$1500 but under \$2400 to program Zefa. 
Thus, more money is allocated to the program with the larger number of beneficiaries (Zefa), but individual people from the smaller program (Alpha) still get more money. 
This type of response is indicative of a compassion fade effect \cite{butts2019helping}.

\item The \emph{\textbf{majority-skewed allocation}} $\in (2400,3000]$ strategy favours the cause with more beneficiaries, indicating that the participant has donated at least over \$2400 up to the maximum amount, \$3000 to program Zefa. 
Thus, more money is allocated to individual people in the charity program with the larger number of beneficiaries (Zefa). 
The allocation favors both the larger program and the individual people in this program.

\end{itemize}




% Since our experiment consists of participants allocating \$0 to \$3000 between the two charity programs, we measure amount of money allocated to the larger of the two charity programs, \emph{Zefa}.
% This program choice is arbitrary as gaining the amount donated to program \emph{Alpha} would simply mean subtracting \$3000 from our measure for all participants.
% We further classify our measure into each of the five strategies described below.



==> archives/archive-with-comments-Sep14/05-study1.tex <==
\section{Experiment 1: Initial Investigation of Resource Allocation}

Since no prior studies have looked at visualization framing in the context of charitable resource allocations, we designed this first experiment to investigate which donation strategies people follow when presented with text and visualizations with different framings. Informed by prior studies in psychology, we also set out to verify whether effects resulting from cognitive biases such as drop-in-the-bucket \cite{friedrich2010individual} or compassion fade \cite{butts2019helping}, would hold within our study design. Specifically, our research questions for this experiment were:
\begin{itemize}
    \item \textbf{RQ1.1} To what extent does a visual representation of information affect donation allocations compared to a design with the same information presented as text only?
    \item \textbf{RQ1.2} To what extent does framing the donation amount per individual affect donation allocations when compared to framing the donation amount per program?
    \item \textbf{RQ1.3} To what extent do the factors of information representation and information framing interact with one another regarding donation allocations?
    \item \textbf{RQ1.4} The auxiliary research question was to find out what are the most common stated reasons for the donation allocations?
\end{itemize}


\subsection{Experimental Design}
Experiment 1 followed the procedure as described in \autoref{sec:expe-design}. The Alpha and Zefa programs aided 3 and 12 children respectively. The amount to allocate was USD\$3,000, which was deemed reasonable for programs of that scale.  % We chose this allocation amount as we though it provides a realistic amount which charities may use when dealing with budget restrictions for different causes, for programs of the scale of that presented in our scenario.

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/Exp1-conditions.pdf}
    \caption[]{Experiment 1: Screenshots of the stimuli, for our four conditions in respectively.}
    \label{fig:exp_1_conditions}
\end{figure*}


Our between-subject design manipulated \textsc{Presentation-Format} -- the same information was either conveyed using using text only (\textit{text}), or both text and visualization (\textit{text+vis}); and \textsc{framing} of both of these presentation formats -- the same information was presented with either a focus on splitting resources between causes (i.e. \textit{group} framing), or a focus on splitting resources between individuals in the causes (i.e. \textit{individual} framing). See \autoref{sec:tool}. Our full factorial design \textsc{Presentation-Format} \{\textit{text+vis, vis}\} $\times$ \textsc{framing} \{\textit{individual, group}\} resulted in four conditions. The content presented in the display component (see \autoref{fig:interface}-b) of the tools for each condition is depicted in \autoref{fig:exp_1_conditions}.

\subsection{Participants}
Our target sample size was 256 participants, so approximately 64 per condition (participants were randomly assigned a condition at sign up). This gives us a 0.8 power to detect a ``medium'' Cohen d’s effect size of 0.5 between any two conditions, as computed by the G*Power software for differences between independent means. Out of the 256 participants who consented, 17 were excluded for not completing the study or failing at the attention check. The 239 remaining responses were divided as follows: 63 were assigned the \emph{(text+vis, individual)} condition, 63 completed the \emph{(text, individual)} condition, 56 completed the \emph{(text+vis, group)} condition, and 60 completed the \emph{(text, group)} condition.

\subsection{Measurements \& Analyses}
\label{sec:exp1-analysis}
We performed the measurements and analyses as described in Sections \ref{sec:measurements} \& \ref{sec:analyses}. We used the allocation to the larger group Zefa as a way to measure (un)fairness: a value of 2400 corresponds to a fair allocation, and the further the distance to this value, the more unfair the allocation.

For the qualitative coding of free-from justification comments, we followed an emergent coding approach \cite{stemler2000overview}: four coders independently assigned labels to participant responses. One coder did so across all responses while the three other coders each covered a separate one-third of the responses. All coders were blind to other data to any information which might supplement the participant's response, such as the amount they allocated to each program. All coders then discussed respective codes, refining, combining, and merging codes where appropriate, converging on a common consolidated coding scheme comprising of 5 categories, each of which comprising several codes (see Supplemental for initial and consolidated codes). One coder re-coded all shuffled responses using the new scheme.

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/Exp1-summary-results.pdf}
    \caption[]
    {Results of Experiment 1: (a) Distribution of allocation strategy chosen by participants, by \textsc{Presentation Format} and \textsc{Framing} (see \S \ref{sec:tool}). (b) Mean allocation granted to Zefa (i.e. mean Large Program Allocation Amount) by condition. Error bars are 95\% CIs.}
    \label{fig:exp_1_summary}
\end{figure*}

\subsection{Results}
\autoref{fig:exp_1_summary} shows a summary of our results by condition. The stacked bar chart (\texttt{a}) shows a break down of responses per allocation strategy (see \S \ref{sec:analyses}), and the error bars (\texttt{b}) show 95\% CIs of mean donation allocations to Zefa, compared to a fair allocation (\$2400).

Overall, most participants opted for a fair allocation strategy. \autoref{fig:exp_1_summary}-b shows mean allocations to Zefa nearing or covering the \$2,400 value. \autoref{fig:exp_1_summary}-a shows that the condition with fewer participants choosing a fair allocation (in light blue) was the one with textual information and group framing (40\% of participants), while showing text+visualization with individual framing led to 78\% fair allocations. Also, a considerable amount of participants chose a mixed allocation strategy in group framing conditions (min: 12\% for \textit{(text+vis,individual)}, max: 34\% for the \textit{(text+vis, group)} condition), which shifted the CIs of those conditions farther from the fair allocation threshold. Below, we discuss our results organized by research question.
% The mixed allocation (in gray) and the majority-skewed allocation (dark blue) where the two next preferred strategies for all conditions \flag{More details here?}. 

\textbf{RQ1.1: Effect of Adding a Visualization Support.} We were interested in learning the extent to which different presentation formats affect resource allocation. \autoref{fig:exp1-detailed-results}-a shows the effect of supplementing text with a visualization on our metric, by framing. We find no evidence to support the claim that the addition of a visualization affects allocation fairness when compared to a design with the same information presented as text only, as both CIs spread around zero.


\textbf{RQ1.2: Effect of Framing.} We were interested in learning the extent to which different framings affect resource allocation. \autoref{fig:exp1-detailed-results}-b shows the effect of varying framing on our metric, for each presentation format. Overall, we find weak evidence suggesting that an individual framing leads to fairer resource allocations than a group framing. This piece of evidence is clearer for the condition where both textual and visual information is available (\$-105, CI [-214, -6]). % We find evidence that for the \textit{(text+vis)} presentation format, donations to Zefa tend to be higher when the framing is focused on \textit{individual} than when it is focused on \textit{group}. This finding, combined with visual inspection of \autoref{fig:exp_1_summary}, suggests that there is a weak evidence that when a supplementing visualization is present, participants tended to allocate more fairly when information was presented with an \textit{individual-}focused framing than with a \textit{group-}focused framing. Since the CI for the \textit{text} condition spreads around zero, we also conclude that there no evidence that an individual-focused framing affects fair allocation when compared to a group-focused framing for this presentation format.

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/Exp1-detailed-results.pdf}
    \caption[]
    {Results of Experiment 1: Effect of \textsc{Presentation Format} (a) and \textsc{Framing} (b) on the \flag{allocation fairness metric (Large Program Allocation Amount)}, and interaction between our different factors (c). Error bars are 95\% CIs.}
    \label{fig:exp1-detailed-results}
\end{figure*}

\textbf{RQ1.3: Interaction between text framing and visual representation.} We were interested in learning the extent to which different design factors (i.e. presentation format and information framing) interact with one another regarding donation allocations. \autoref{fig:exp1-detailed-results}-c shows such interaction. We find no evidence that our factors interact with one another with respect to resource allocation. %Since it is hard to interpret non-crossover interactions, we will conclude only \flag{if we find a crossover interaction} \cite{wagenmakers2012interpretation, krzywinski2013error}.

\textbf{RQ1.4: Auxiliary Question - Stated Reason} We were also interested in finding out what are the most common stated reasons participants provide for their donation allocations. To do so, we coded the free-form justifications (see \S \ref{sec:exp1-analysis}). Our main insights from this process are as follows:

(i) We found inconsistencies between the strategy used by some participants and their justification. The \emph{sense of equality} code determined if participants responses indicated that they tried to allocate equitably across charities. We coded 70 responses as such (out of 239), however 12 of those participants did not use a fair strategy when allocating resources between the programs. 

(ii) Free-text responses suggest that mental calculations (e.g. dividing a total amount by number of beneficiaries) are not necessarily performed to achieve a fair allocation, and are prone to errors. The \emph{math} code category indicated whether the response included some explicit calculation. Of the 44 participants who did include such mention, eight did not use the fair allocation strategy.

(iii) Some participants made assumptions about the programs, which have likely impacted their response. The \emph{contextual influence} code category determined whether the response indicated that the participant's allocation was chosen based on personal interpretations of the scenario, e.g. presuming that program Zefa solves a more significant problem whereas our scenario did not state so. This finding motivated us to reword the scenarios in subsequent experiments, to leave less room to such extrapolations. 

(iv) The two other coding categories did not provide additional insight, and are thus omitted in interest of space. 

\textbf{Additional Analysis.} 


%The difference in means between showing information focusing on donations for individuals (\emph{personFraming}) and focusing on donations for the groups (\emph{causeFraming}) for each of the two presentation formats is shown in Figure \ref{fig:exp_1_dom_framing} to help us answer research question 1.2. 

%Since there is overlap between the confidence intervals, we find little evidence that framing the donation amount per individual affect donation allocations when compared to framing the donation amount per program.

%However when looking at the distributions of responses (i.e. the amount of money allocated to the Zefa program) for each of the four conditions as per Figure X, we see no distinct value for either strategy as a prominent alternative to donating \$2400.

%To gain a sense of general strategies used by participants in each condition for an allocation, we can observe Figure X which shows the proportions of responses per each allocation strategy, for each of the four conditions.


%Note that for all conditions, 
%The 95\% confidence intervals and point estimates for the amount allocated to Zefa for each of the four conditions is shown in Figure X. 


\subsection{Discussion}

Contrary to our expectations, the presentation format used does not seem to greatly affect resource allocations. We could not find evidence that supplementing text with a visualization produces a fairer resource allocation. If this result turns out to be true, it refutes our initial assumption that showing a visual representation would help participants to evenly distribute the available resources. On the other hand, it also means that using a visualization to complement text might not negatively affect the allocation fairness.

Our findings also suggest that the way the information is framed can affect how people allocate resources. We found weak evidence that presenting information through an individual framing influenced participants to perform fairer allocations when compared to a group framing. We suspect that by presenting information about the exact amount that each individual would receive influenced participants to choose a value that would help everybody equally. This finding contributes to better understand the differences between those two types of framing and reinforces previous evidence \cite{TODO} that information framing can play a role on decision-making.

We later realized that the weak evidence for the effect of information framing could have been caused by the metric that we used. Mean allocation and mean differences are sensitive to extreme values. Therefore, the majority-skewed responses could have pushed the mean closer to 2400, even in the conditions that participants had a smaller proportion of fair allocations. We decided to re-interpret the same data with another metric as part of a supplementary analysis. We used the proportion of fair allocations, which consists of dividing the number of fair allocations by the number of unfair allocations in each condition. This new metric is less sensitive to extreme values and reflects more our research aim of exploring fair allocations. Investigating the proportion of fair allocations, we did find clearer evidence that individual framing is more effective than group framing for influencing participants to allocate fairly. However, as this unplanned analysis was not preregistered, we decided to replicate our first experiment to confirm our initial findings with this more robust metric.

% We note though, that for the \textit{(text, group)} and \textit{(text+vis, group)} conditions, CI ranges are slightly lower than \$2,400, suggesting a potential effect of framing on allocation fairness.

% \flag{
%Mentioned we conducted supplementary analysis -- elaborate further. Relate back to why we changed the measurements.
%Experiment 1 that participants responses were largely a fair allocation between the two programs. 
%We also found through further unplanned analysis some evidence that proportion of unfair allocation varied across different conditions, possibly with effect sizes that are stronger than the difference in means. We conducted this second experiment to confirm this tentative finding.
% }

% \flag{
%Before the start of the study, we expected \emph{groupFraming} would lead lower fair allocations as a strategy, however we found that this was not the case.
%The fair strategy seems to have been the dominant majority in all conditions, however we did see less fair allocations in the condition with \emph{groupFraming}.
% }

% \flag{
%These small differences might be likely due to a majority of participants across all conditions choosing a fair allocation.
%In conditions where less people allocated \$2400, the remaining allocations were both smaller and larger than \$2400, canceling out the effects when aggregated as a mean.
%In other words, we initially expected that effects such as compassion fade would lead more people to choose naive and mixed allocations in some conditions ($<$ \$2400), which would push the mean donation lower, but this effect seems to have been canceled out by larger-than-anticipated proportion of people choosing majority-skewed allocations ($<$ \$2400).
% }

% \flag{
%Since we find no evidence for any type of interaction or difference of means it is difficult to judge how much influence framing visualizations can have.
%This could mean there minimal influence of cognitive biases which hindering the participants ability to donate fairly, depending on framing or the presence of a visualization.
%There may have been other effects and strategies at play which also led to greater donation, and as such, since compassion fade was likely not the only effect present, mean donation to Zefa was insufficient to measure and understand differences in allocation strategies.
% }

% \flag{
% \arnav{talk about content analysis as well here}
%After conducting Experiment 1, which focused on differences in mean allocation, we found that the differences in mean allocation were small across conditions, resulting in mostly inconclusive findings.
% }



==> archives/archive-with-comments-Sep14/06-study2.tex <==
\section{Experiment 2: A Closer Look at Fair vs. Unfair Allocations}

%We learned from Experiment 1 that participants responses were largely a fair allocation between the two programs. We also found through further unplanned analysis some evidence that proportion of unfair allocation varied across different conditions, possibly with effect sizes that are stronger than the difference in means. 
We conducted this second experiment to replicate the first experiment with a more robust metric to confirm the previous findings. We also made minor changes to the scenario brief based on observed limitations from Experiment 1. Our main research questions were:

\begin{itemize}
    \item \textbf{RQ2.1} To what extent does a visual representation of information influence the proportion of fair allocations compared to a design with the same information presented as text only?
    \item \textbf{RQ2.2} To what extent does framing the donation amount per individual influence the proportion of fair allocations when compared to framing the donation amount per program?
\end{itemize}

\subsection{Experimental Design}
The same procedure and design as that of Experiment 1 was used. The only difference was in the scenario brief. To prevent participants speculating on the programs' respective effectiveness, we added context in the brief: (i) a description of needs (i.e., \textit{``Children from both programs are in a very similar situation and need money equally. They will not benefit from any other donation than yours.''}), and (ii) a clarification of how the money will be allocated within the programs (i.e. \textit{``All the money you donate to a program will be split evenly between the children in the program.''})

%There were no changes in the experimental design from the first experiment.
%We similarly conduct a 2x2 fully-crossed between-subject factorial design manipulating the \emph{Presentation format} and \textsc{Framing} independent variables, as described in Experiment 1.
%The allocation design and dependant variable of this experiment remains the same to Experiment 1 as we capture fairness indirectly through the Large Program Allocation measure, i.e allocation towards Zefa.

%There were no significant changes in the procedure from experiment 1 except on page 3, where the participant read the story.
%In this page, we additionally clarify the assumptions behind our allocation scenario by providing the following extra instructions:
%\begin{itemize}
%    \item All the money you donate to a program will be split evenly between the children in the program
%    \item Children from both programs are in a very similar situation and need money equally. They will not benefit from any other donation than yours
%\end{itemize}
%We specify a these constraints for the participant as it helps alleviate partial confusion about the effectiveness of both programs found within the coded responses of Experiment 1.

\subsection{Participants}
Like for Experiment 1, we targeted a sample size of 256 ($\sim$ 64 per condition). Twelve (12) participants were excluded. The 244 remaining responses were divided as follows: 62 in the \emph{(text+vis, individual)} condition, 63 in the \emph{(text, individual)} condition, 54 in the \emph{(text+vis, group)} condition, and 65 in the \emph{(text, group)} condition.

%Since we has no changes in the design of the conditions, our target sample size was N = 256 participants, approximately 64 per condition, the same as experiment 1.

%All screening and pre-screening procedures were kept the same as Experiment 1.
%Out of the 256 contributors who agreed to the consent form, 244 passed the attention check or did not drop out of the study, meaning an attrition rate of 4.7\% (N = 12).

%Participation for each condition was divided as follows: 62 participants for the \emph{(text+vis, individual)} condition, 63 participants for the \emph{(text, individual)} condition, 54 participants for the \emph{(text+vis, group)} condition  and 65 participants for the \emph{(text, group)} condition.

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/Exp2-summary-results.pdf}
    \caption[]
    {Results of Experiment 2: (a) Distribution of allocation strategy chosen by participants, by \textsc{Presentation Format} and \textsc{Framing} (see \S \ref{sec:tool}). (b) Mean proportion of people making a fair allocation by condition. Error bars are 95\% CIs.}
    \label{fig:exp_2_summary}
\end{figure*}


\subsection{Measurements \& Analyses}
Unlike in Experiment 1, here we used the relative proportion of people who chose to use a fair allocation strategy as a means to assess allocation (un)fairness.
While we report descriptive statistics showing the break down of responses per allocation strategies using all five strategies from \autoref{sec:measurements}, we decided against performing inferential statistics at this level of granularity. Rather, we focus on fair vs. unfair responses. 
%The reasons are that we were mostly interested in verifying the effect of tool designs on fair vs. unfair allocation, and also because too few participants chose 

%the proportion of people who chose to use an unfair responses with respect to sub-categories. The reasons are that we were mostly interested in verifying the (which does not 

%Relatively few participants used other strategies besides 
%In this experiment, we focused on the proportion of people who chose to use a fair allocation strategy (\$2400) towards Zefa compared the total allocation overall (see \S \ref{??}).
%Note that we could have subdivided the unfair allocation into the four sub strategies we identified for experiment 1, but since we observed that relatively few participants used any sub-strategy which unfair allocation was divided into, this would probably result in a too low statistical power.
%This would also result in more tests, raising multiplicity problems.
%So, in order to find greater statistical power within our analysis, we only find the proportional difference between the fair and unfair strategies.
%\flag{However, specifically for Experiment 2, we plot using the proportion of fair responses for a condition compared to all other responses in that condition.} \fanny{What does this mean? I don't understand}
%\flag{We performed the measurements and analyses as described in Sections \ref{sec:measurements} \& \ref{sec:analyses}. We used the mean allocation to the larger group Zefa as measure of unfairness, where a value of 2400 corresponds to a fair allocation.}


\subsection{Results}
\autoref{fig:exp_2_summary} shows a summary of our results for each condition.
The stacked chart on the left shows a break down of responses per allocation strategy, by condition (\S \ref{sec:measurements}). The plot on the right shows the mean proportion of fair allocation with respect to all responses within each condition.



Both plots suggest that most participants performed a fair allocation. We observe that individual-framing conditions tend to result in slightly higher proportions of fair allocations compared to group-framing ones.% -- with \flag{66\%} (mean: 0.66 {\small CI[0.54,0.78]}), \flag{71\%} (mean: 0.71 {\small CI[0.60, 0.82])}, \flag{54\%} (mean: 0.54 {\small CI[0.42, 0.66]}), \flag{57\%} (mean: 0.57 {\small CI[0.44, 0.71]}
%respectively. 
Potential effects are further investigated under our research questions below.

%While the range of the bootstrapped confidence intervals vary by 0.4 between the min and max values, inspecting the bar chart indicates that there was only approximately a difference 0.1 (i.e 10\%) proportional of fair allocations between all conditions in the preformed experiment.

%%% PREVIOUS VERSION %%%%%%%
%The plot on the right shows the proportion of people who allocated fairly to program Zefa for each condition, i.e. participants who allocated \$2400 compare to all participants in the condition, with 95\% bootstrapped confidence intervals.
%Both plots indicate that most participants performed a fair allocation (min: \flag{0.40} proportion of participants for \flag{xx}, max: \flag{0.8} proportion of participants for \flag{xx}). 

%\flag{Contrasting with Experiment 1, we note that the proportion of fair allocations across each condition was much closer to one another}. \fanny{I don't understand, and that's not the metric we had here}
%While the range of the bootstrapped confidence intervals vary by 0.4 between the min and max values, inspecting the bar chart indicates that there was only approximately a difference 0.1 (i.e 10\%) proportional of fair allocations between all conditions in the preformed experiment.
%We also note that condition with the lowest proportion of fair allocations (i.e \emph{(text, group)} in Experiment 1, had higher fair allocations in this experiment however the condition with the highest proportion of fair allocations (i.e \emph{(text+vis, person)}), had lower fair allocations.

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.8\textwidth]{figures/Exp2-detailed-results.pdf}
    \caption[]
    {Results of Experiment 2: Effect of \textsc{Presentation Format} (a) and \textsc{Framing} (b) on overall proportion of fair allocations made. Error bars are 95\% CIs.}
    \label{fig:exp_2_analysis}
\end{figure*}

\textbf{RQ2.1: Effect of Adding a Visualization Support.}
We were interested in investigating the effect of presentation format on resource allocation. \autoref{fig:exp_2_analysis}-a shows the difference in proportions between the \textit{text} format and the \textit{text+vis} format for each of the two framings. The effect seems to be negligible, independently of framing. 

%Both CIs are slightly to the right of zero, meaning \emph{text+vis} presentation format  marginally promoted fairer allocations than text only presentation.
%We note that the confidence intervals overlap closely, with minimal difference between the means. 
%Since both intervals intersect zero, we find no evidence to support the claim that presentation format influences resource allocations.

\textbf{RQ2.2: Effect of Framing.}
We were interested in investigating the effect of information framing on resource allocation. \autoref{fig:exp_2_analysis}-b show the difference in proportion of fair allocations between \textit{individual} and \textit{group} framing, by presentation format. There is weak evidence that individual framing motivates fairer allocations than group framing in both presentation formats ((mean: -0.13 {\small CI[-0.32,0.03]}) for text+viz, (mean: -0.12 {\small CI[-0.28, 0.05]}) for text).


%meaning that we find no evidence to support the claim that information framing influences resource allocation. However, we note that
%Both intervals are slightly to the left of zero, meaning individual framing promoted fairer allocations than group framing however only marginally.
%Similar the previous condition, the confidence intervals also have a significant overlap. %Since both intervals intersect zero, we find no evidence to support the claim that information framing influences resource allocation.

\subsection{Discussion}

The findings from this experiment are in line with the results from experiment 1. First, results suggest that supplementing text with a visualization seems to produce the same proportion of fair allocations than using only text. Second, we found weak evidence that individual framings seem to be more effective for motivating fair allocations than group framings, in both presentation formats. Those results strengthen the assumption that information framing plays a major role on resource allocation compared to presentation format.

The higher variation of fair allocations across conditions in the previous experiment was not reproduced in this experiment (compare \autoref{fig:exp_2_summary}-a and \autoref{fig:exp_1_summary}-a). As previously mentioned, maybe some instructions in the first experiment led participants to believe that a specific program was more important than the other, which caused a greater variance in responses. The instruction improvements in this experiment may have reduced room for assumption regarding program effectiveness, explaining the lower variation.


\flag{To gain a better understanding of the role of each component and framing used alone or in conjonction, in the following experiment below, we examine each pair (presentation format, framing) in isolation, allowing us to look at congruence and uncongruence of framings.}

==> archives/archive-with-comments-Sep14/07-study3.tex <==
\section{Experiment 3: A Rigorous Look at Information Framing}
% Methods increasing proportion of participant size, fairness metric and 

The previous experiments investigated whether \emph{supplementing} text presentation with a visualization influenced fair allocation. In this experiment, we take a closer look at the role of information framing, exploring each presentation format independently (i.e text only, visualization only, and text together with visualization). This allows us to isolate the role of presenting information through visualization only, since Experiments 1 \& 2 always included text, with or without a supplementing visualization. Prior studies found little influence of visualizations in inducing prosocial behaviors (\S \ref{sec:related_work}). In Experiment 3, we set out to validate whether visualizations can substitute text, while promoting a similar propensity for fair allocations in our context.

This also allows us to examine conditions where text and visualization have incongruent framings (e.g. text focuses on individuals and visualization focuses on group, and vice-versa, see \S \ref{sec:tool}). Experiment 1 \& 2 only included congruent framings (with additional caveat that text presentation included both group and individual framings in the individual-focused framing design).

Our main research question focused on the effect of visualization framing as follows:
\begin{itemize}
    \item \textbf{RQ3.1} To what extent does visualization framing influence the unfairness of fund allocations across all text framing conditions? 
\end{itemize}
Secondary research questions aimed at uncovering the effect of visualization framing were as follows:
\begin{itemize}
    \item \textbf{RQ3.2} To what extent does visualization framing influence the fairness of allocations when
    \textbf{(a)} no numerical information is present;
    \textbf{(b)} numerical information is shown with a group framing;
    and when \textbf{(c)} numerical information is shown with a person framing?
    \item \textbf{RQ3.3} Does the effect of visualization framing depend on numerical framing?  
    % (visually compare the overlap between the CIs for the three simple effects previously listed.)
\end{itemize}
An additional secondary research question focused on examining the effect of presenting a visualization:
\begin{itemize}
    \item \textbf{RQ3.4} To what extent does the presence of visualization influence the fairness of allocations when
    \textbf{(a)} the numerical information and visualization have a congruent group framing;
    \textbf{(b)} the numerical information and visualization have a congruent person framing;
    and when \textbf{(c)} the numerical information and visualization have an incongruent framing?
\end{itemize}
Finally, our two auxiliary research questions were as follows:
\begin{itemize}
    \item \textbf{RQ3.5} What are the most common stated reasons for the donation allocations?
    \item \textbf{RQ3.6} How does each condition affect the duration taken to complete an allocation choice?
\end{itemize}

\subsection{Experimental Design}

We followed the procedure described in \ref{sec:procedure}. The program \emph{Alpha} had 3 children. We changed the size of the program Zefa to now include 120 children, resulting in a 1:40 ration (instead of 1:4 in the other Experiments). Since a larger difference between the programs might be more prone to the compassion fade bias, this will allow us to further examine the robustness of our previous findings.

We also changed the amount of the resource to be allocated accordingly. Keeping a target \$200 per individual for a fair allocation, the total amount to be allocated was changed from \$3000 to \$24,600.

Finally, we made subtle refinements to the design of our interface and visualization, i.e. opting for a dark theme (i.e. black background) to achieve higher contrast, and traded the stacked coins pictogram for a simple yellow circle for increased simplicity and readability.

We ran a within-subject experiment were we manipulated the presence and framing of both a text and a visualization presentation format as follows. The \textsc{Text-Framing} specifies the framing employed for the text presentation format: \textit{textGroup} uses a group-focused framing only; \textit{textIndividual} uses an individual-focused framing only; and \textit{textNone} means that text presentation is not included. Similarly, the \textsc{Visualization-Framing} independent variable manipulates framing of the visual representation of information, weith \textit{visGroup} and \textit{visIndivudal} values corresponding to a group and an individual framing respectively, and \textit{visNone} corresponds to no visualization at all.

The full factorial design \textsc{Visualization-Framing} \{\textit{visNone, visGroup, visIndividual}\} $\times$ \textsc{Text-Framing} \{\textit{textNone, textGroup, textIndividual}\} results in nine conditions. However, we discard the \emphb{(textNone, visNone)} condition as it results in an empty display (i.e. no information is presented at all). The stimulus included in the display component of the interactive tools (\autoref{fig:interface}-b) for all conditions respectively are depicted in \flag{\autoref{fig:exp_3_conditions}}. \flag{Figure: TODO}.




%While the allocation design used in Experiments 1 and 2 (\autoref{fig:exp_1_conditions}) promoted the fair allocation strategy irrespective of the condition, the role that visualizations played in influencing such behaviour was unclear.
%All conditions previously included text even in the presence of a visualization. 
%Thus, participants may have been neglecting the visualization altogether and relying solely on text, leading to the minimal difference in proportion of fair allocations across each condition, as seen in Experiment 2.
% Since prior work in similar contexts has shown little influence of visualizations (see \S \ref{sec:related_work}) in inducing prosocial behaviours, we wanted to validate whether visualizations can replace text while promoting a similar propensity for fair allocations.
%Even though it may be the case that visualizations promote similar allocation behaviour as text, the addition visualizations in resource allocation tools may have other benefits unrelated to fair allocations.

%In our previous design, the individual framing in the text representation also contained the text from the group framing. 
%However, this would make it difficult to understand which part of the text representation our visualization could be comparable to.
%As such, we split our text representation such that the content of individual and group framing did not overlap.

%Overall, in Experiment 3 we granularized the content presented between different framings for the text representation and further investigate the utility of visualizations. 


\subsection{Measurement \& Analysis}

We performed the measurements and analyses as described in Sections \ref{sec:measurements} \& \ref{sec:analyses}. To gauge allocation (un)fairness, we define the \textit{unfairness distance} (\texttt{UFD}) as the distance to a fair allocation, in dollars. A value of zero for this metric means a fair allocation has been made. The further from zero, the unfairer the allocation. For instance, a \texttt{UFD} value of \$600 means that either \$24,600 or \$23,400 has been allocated to Zefa, both of which are a distance of \$600 away from a fair allocation (which is \$24,000 to Zefa).

Note that our \texttt{UFD} metric is comparable to the standard Gini index~\cite{gini1997concentration}, which could be seen as a normalized form our metric.
We use \texttt{UFD} as we wanted to use a metric which preserves our exact allocation value for both programs as specific breakpoints might derive additional meaning in the context of our allocation strategies. 

\subsection{Participants}

Our target sample size was 512 participants ($\sim$ 64 per condition), giving us the same Cohen d’s effect size between any two conditions. Seventeen (17) participants were excluded (attrition rate: 3.3\%). The 495 valid responses were distributed across conditions as per \autoref{table:exp3_particpant}.

\begin{table}[h]
{\scriptsize
\centering
\begin{tabular}{c c c} 
\textbf{Text Framing} & \textbf{Visualization Framing} & \textbf{Participants} \\  [0.5ex]
\hline
textGroup & visNone & 60 \\ 
texttextIndividual & visNone & 64 \\
textNone & visGroup & 68 \\
textGroup & visGroup & 52 \\
textIndividual & visGroup & 50 \\
textNone & visIndividual & 73   \\
textGroup & visIndividual & 73 \\
textIndividual & visIndividual & 55 
\end{tabular}
}
\caption{Experiment 3: Participant count for each condition}
\label{table:exp3_particpant}
\end{table}


%Out of the 512 contributors who agreed to the consent form, 495 passed the attention check and completed the experiment to the end, giving an attrition rate of 3.3\% (N = 17).
%Participation for each condition was divided as per \autoref{table:exp3_particpant}.

%Having a \texttt{UFD} of 0 would mean a fair allocation has been made, i.e  \$24,000 has been allocated by a participant to program Zefa in Experiment 3.
%However, the further from zero, the unfairer the allocation. For example, a value of \$600 \texttt{UFD} could mean \$24600 or \$23,400 has been allocated to Zefa, both of which are a distance of 600 away from a perfectly fair allocation which is \$24,000.

%Point estimates and confidence intervals corresponding to secondary research questions will also be reported, but any finding will be qualified as tentative due to statistical multiplicity issues.

% All results were measured in the \textbf{unfairness distance} (\texttt{UFD}) metric.
% We define allocation unfairness as the distance to the fair allocation, i.e., the absolute difference between the participant's donation to Zefa and the fair donation amount of \$24 000, as described in section \flag{\ref{?}}. 
% \flag{}

%\subsection{Procedure}
% Every participant read the same story experiment 2 however the ratio of children between the two program will different, with program \emph{Alpha} having 3 children while program Zefa now including 120 children. 
% Unlike the previous experiments, instead of a ratio of 1:4, we have a ratio of 1:40 between Alpha and Zefa.
% This is done to make sure our findings from the previous experiment were robust to proportional increases, which may lead to an increase the compassion fade effect.

%Since we wanted the amount allocated for each individual to stay the same (i.e \$200 per individual), the total amount specified to be allocated in the story changed from \$3000 to \$24600.
%\flag{Write Strategies here (see how sec 4 looks)}

%The visual design in our \emph{visualization} presentation format was also changed from experiments 1 and 2 as shown in \flag{\autoref{fig:exp_3_conditions}} to create more abstract representations for the coin marks.
%Due to the changes in the color design, we added ensured a high contrast color scheme, in relation to the visualization and it's background color.

%The numerical component was at the top of each panel and always showed the name of the program.
%Unlike previous experiments, it showed the number of beneficiaries and current donation amount for the program if the user had a \emph{textGroup} condition and only the amount received per person in the \emph{textIndividual} condition.
% \subsection{Analyses}
% We performed inferential statistics and draw our inferences from graphically-reported point and interval estimates \cite{cumming2005inference}. All effects are estimated by using the percentile method of obtaining 95\% bootstrapped confidence intervals and any differences are done through statistical contrast \cite{kirby2013bootes}.
% We also do not adjust for multiplicity. Point estimates and confidence intervals corresponding to secondary research questions will also be reported, but any finding will be qualified as tentative due to statistical multiplicity issues.

% We also plot the mean allocation unfairness for each of the eight conditions, with 95\% bootstrap confidence intervals (CIs).
% Similarly as the first two experiments, these individual means estimates will be reported for information purposes and will not be directly used to draw conclusions.

% All results were measured in the \textbf{unfairness distance} (\texttt{UFD}) metric.
% We define allocation unfairness as the distance to the fair allocation, i.e., the absolute difference between the participant's donation to Zefa and the fair donation amount of \$24 000, as described in section \flag{\ref{?}}. 

% \subsection{Participants}
% \begin{table}[h]
% {\scriptsize
% \centering
% \begin{tabular}{c c c} 
% \textbf{Text Framing} & \textbf{Visualization framing} & \textbf{Participants} \\  [0.5ex]
% \hline
% textGroup & visNone & 60 \\ 
% textIndividual & visNone & 64 \\
% textNone & visGroup & 68 \\
% textGroup & visGroup & 52 \\
% textIndividual & visGroup & 50 \\
% textNone & visIndividual & 73   \\
% textGroup & visIndividual & 73 \\
% textIndividual & visIndividual & 55 
% \end{tabular}
% }
% \caption{Participant count for all conditions}
% \label{table:exp3_particpant}
% \end{table}
% Our target sample size was N = 512 participants, so about 64 per condition, the same amount per condition as Experiments 1 and 2. This gives us the same Cohen d’s effect size between any two conditions.
% Study platform, screening procedures, and pre-screening procedures were kept the same as past experiments.
% Out of the 512 contributors who agreed to the consent form, 495 passed the attention check and completed the experiment to the end, giving an attrition rate of 3.3\% (N = 17).
% Participation for each condition was divided as per \autoref{table:exp3_particpant}.



\begin{figure*}[h]
    \centering
    \includegraphics[width=\textwidth]{figures/Exp3-summary-results.pdf}
    \caption[]
    {Results of Experiment 3: (a) Distribution of allocation strategy chosen by participants, by \textsc{Text Framing} and \textsc{Visualization Framing}, and (b) Mean measure of unfairness per condition. Error bars are 95\% CIs.}
    \label{fig:exp_3_summary}
\end{figure*}


\begin{figure*}[h]
    \centering
    \includegraphics[width=\textwidth]{figures/Exp3-detailed-results.pdf}
    \caption[]
    {Results of Experiment 3: \flag{xxx}. Error bars are 95\% CIs.}
    \label{fig:exp_3_analysis}
\end{figure*}


\subsection{Results}
\autoref{fig:exp_3_summary} shows a summary of our results by condition.  The stacked bar chart on the left shows a break down of responses per allocation strategy by condition.
The right plot shows the mean unfairness measurement per condition. From \autoref{fig:exp_3_summary}-a, we note that fair allocations were not a majority in all conditions, suggesting potential effects in this more granular experimental design, which we investigate through our research questions as follows.

\textbf{RQ3.1: Effect of Visualization Framing.}
We were interested in learning the extent to which visualization framing (visGroup vs. visIndividual) influences the unfairness of allocations across all text framing conditions.
\autoref{fig:exp_3_analysis}-a shows the difference in mean allocation unfairness corresponding to the following contrast of our conditions:\\
{\small\textit{
\{(textNone, visGroup) $\cup$ 
(textGroup, visGroup) $\cup$ 
(textIndividual, visGroup)\}
--\\
\{(textNone, visIndividual) $\cup$
(textGroup, visIndividual) $\cup$
(textIndividual, visIndividual)\}
}}\\
This represents the influence of visualization framing across all text framing conditions.
We found very weak evidence (mean: \$610 {\small CI[-295, 1576]}) that group framing for visualizations might cause more unfairness in allocations when compared to a person framing for visualizations.

\textbf{RQ3.2: Effect of Presenting Visualization Framing.}
We were interested in learning to what extent does visualization framing influence the fairness of allocations across all values in \textsc{Text-Framing}.
\autoref{fig:exp_3_analysis}-b shows the difference in unfairness between \textit{visGroup} and  \textit{visIndividual} when presented with \textit{textNone}, \textit{textGroup}, \textit{textIndividual} framing.

To find the influence of visualization framing when \textit{noText} framing is present (RQ3.2a), we contrast the conditions $\small{\emph{(textNone, visGroup)} - \emph{(textNone, visIndividual)}}$. To find the influence of visualization framing when numerical information is shown with an \textit{individualText} framing (RQ3.2c), we contrast the conditions $\small{\emph{(textIndividual, visGroup)} - \emph{(textIndividual, visIndividual)}}$.
Since the CIs for both contrasts cross zero, we find that results are inconclusive and find no evidence that group framing causes more or less unfairness in allocations when compared to a person framing for visualizations, when no text  information is present or when individual text framing is used.

To find the influence of visualization framing when numerical information is shown with a \textit{groupText} framing (RQ3.2b), we contrast the conditions $\small{\emph{(textGroup, visGroup)}} - \small{\emph{(textGroup, visIndividual)}}$.
Since the CI is to the right of zero and does not cross it, we find some evidence that group framing for visualizations cause more unfair allocations than person framing for visualizations, when a group text framing is present, with a mean estimated difference in unfairness of (mean: \$1676 {\small CI[217, 3231]}).

% To find the influence of visualization framing when numerical information is shown with an \textit{individualText} framing (RQ3.2c), we contrast the conditions $\small{\emph{(textIndividual, visGroup)} - \emph{(textIndividual, visIndividual)}}$.
% Since the CI crosses zero, we find that results are inconclusive and find no evidence that group framing causes more or less unfairness in allocations when compared to a person framing for visualizations, when numerical information is present with a person framing.

\textbf{RQ3.3: Overall Effect of Presenting Visualization Framing.}
We were interested in learning to what extent does the effect of visualization framing depend on numerical framing.
To do this, we visually compare the overlap between the CIs in \autoref{fig:exp_2_analysis}-b.
% The results are mostly inconclusive, as there is a fair amount of overlap between confidence intervals between all text conditions.
% Specifically, 
The overlap between the CIs for \textit{textNone} and \textit{textIndividual}; and for \textit{textGroup} and \textit{textIndividual} is too large to be able to conclude in an interaction \cite{krzywinski2013error}.
The overlap between the CI for \textit{textGroup} and \textit{textNone} is relatively small, so there is some weak evidence that visualization framing has a larger effect (i.e, group visualization framing increases unfairness more as compared to individual visualization framing) when group text framing is used than when there no text information is present.

\textbf{RQ3.4: Effect of Presenting Congruent or Incongruent Visualizations.}
We were interested in learning to what extent does the presence of visualization influence the fairness of allocations when there was a framing match or mismatch between text and visualization framing.
\autoref{fig:exp_3_analysis}-c shows the mean difference in unfairness for conditions with strictly congruent or incongruent text and visualization framing.

To find the effect of showing a visualization when the text information and visualization have a congruent \emph{group} framing (RQ3.4a) we contrast $\small{\emph{(textGroup, visNone)} - \emph{(textGroup, visGroup)}}$.
To find the effect of showing a visualization when the text information and visualization have a congruent \emph{person} framing (RQ3.4b) we contrast the conditions $\small{\emph{(textIndividual, visNone)} - \emph{(textIndividual, visIndividual)}}$. As both the CIs for the difference of means cross 0, we cannot claim the influence of congruent group or person framings between visualization and text.

% As both the CIs for the difference of means are cross 0, we cannot claim the influence of a group visualization framing when numerical information with a group framing is present. 

% To find the effect of showing a visualization when the text information and visualization have a congruent \emph{person} framing (RQ3.4b) we contrast the conditions $\small{\emph{(textIndividual, visNone)} - \emph{(textIndividual, visIndividual)}}$.
% We note that there is a negligible gap between the two conditions.
% As the difference of means is extremely close to 0 as well, meaning our bootstrapped CIs cross 0, we cannot claim the influence of congruent person framings.

To find the effect of showing a visualization when text information and visualization have an incongruent framing (RQ3.4c) we find preform two distinct contrasts.
When \textit{textGroup} has an incongruent framing with the visualization, we contrast the conditions $\small{\emph{(textGroup, visNone)} - \emph{(textGroup, visIndividual)}}$.
We find group visualizations cause slightly more unfair allocations  (mean: \$1251 {\small CI[-45, 2664]}). Even though the CIs for the difference of means closely crosses zero, we can claim that there is is an influence of different visualization framings when text information with a individual framing is present.
When \textit{textIndividual} has an incongruent framing with the visualization, we contrast the conditions $\small{\emph{(textIndividual, visNone)} - \emph{(textIndividual, visGroup)}}$.
As the CI crosses zero, we find no evidence that individual framing for visualizations causes less unfair allocations than no visualizations, when a group text framing is present.

\textbf{RQ3.5 \& RQ3.6: Auxiliary research questions}
We were interested in the most common stated reasons for the donation allocations (RQ3.5). 
Since the number of participants using a mixed-allocation strategy differentiated significantly from past experiment, we decided on a further investigation of responses for this category only.
We did an exploratory coding of the responses with 3 codes belonging to one category.
The \emph{zefa cause} code indicated the participant based their justification around giving more to the Zefa cause than to the Alpha cause; the \emph{alpha individual} code indicated the participant based their justification around giving more to the individuals in Alpha than to the individuals in Zefa; and \emph{balanced} code indicated the participant said they gave similar to both programs.  We found that most participants still justified giving more to Zefa due to the higher group size.

To find how each condition affects the duration taken to complete an allocation choice (RQ3.6) we plot the CIs for the mean allocation time for all conditions. 
Most participants donated within 35 to 85 seconds. Observing the CIs for \textit(textNone, visIndvidual) and \textit(textIndividual, visNone), we see that participants in these condition were able to reach a decision the fastest.


\subsection{Discussion}

In this experiment, we took a closer look at the effect of framing. Overall, our findings suggest that individual framings, either for visualization or text, seem to provoke fairer allocations when compared to group framings. This result reinforces the assumption that framing the information in a way that helps donors to identify the amount allocated to individuals motivates them to split the resources equally among all the beneficiaries. We discuss specific effects in more detail.

We found that visualization framing can play a role on resource allocations in specific situations. We found that including an individual-framed visualization is able to curb unfairness compared to group-framed visualizations, when the visual representations are combined with group-framed text. We suspect that the combination of textual information about the groups and an individual framing in visualizations helped participants to identify the amount that each beneficiary would receive, making them to allocate the money more fairly. However, it is important to note that showing visualizations, either individual or group-framed, without an accompanying text made participants to make more unfair allocations. Therefore, it seems that the presence of text is important to influence participants to opt for a fair allocation strategy.

We also found that providing stand-alone text with an individual framing may produce similar fair allocations than including individual-framed visualizations combined with any text framing. However, using group-framed text without including a visualization influences participants to have more unfair allocations. \fix{This finding is important since including visualizations with individual framing did not curb the effect of text framing and also helped to increase the effect of fair allocations when using an incongruent design.} \fanny{It doesn't help but it doesn't harm (even when vis group framing uncongruent with text individual -- but this particular effect is inconclusive) when it's congruent framing -- so we can have a congruent visualization to bring benefits of having visualization} Therefore, incorporating certain visualization framings may bring a net benefit in terms of promoting fairness. This finding adds contrast to prior work within our domain which has limited findings for visualizations which try to influence prosocial behaviours \cite{morais2021can}.


% Overall, this Experiment contained far fewer fair allocations and greater number of mixed allocations than previously observed. This means biases such as compassion fade may have played a stronger role in this Experiment. We also note that generally, a higher unfairness value meant that a higher number of participants used a mixed-allocation. While the number of participants using the \emph{majority-skewed} allocation also grew, we observe that \textit{(textIndividual, visGroup)} condition contained distinctly the lowest number, directly opposing the drop-in-the-bucket effect.
% While we found a weak effect that visualization with an individual framing promotes fair allocations, it is important to note that this effect may have been reduced due to the fact that when no text is present, individual framing for our visualization causes the highest mean unfair allocation. Conversely, when the individual-framed visualization is presented with any text framing, it produces the lowest mean unfair allocations. Since providing stand-alone text with an individual framing also produces approximately the lowest mean unfair allocations as well, we can conclude the framing visualization in an individual framing does not detract from the text. This is important as visualizations might allow other benefits besides improving fairness, thus a finding that certain visualization framings do not cause higher unfairness can be of value.   
%We also find that including an individual-framed visualizations is able to curb unfairness in group-framed text, meaning the incorporating certain framings of visualization may have a net benefit in terms of promoting fairness. This finding adds contrast to prior work within our domain which has limited findings for visualizations which try to influence prosocial behaviours \cite{morais2021can}.

% It is important to note that visualization also provide other benefits.. (put in general discussion)
% The \emph{unfairness} values for conditions \textit{(textIndividual, visNone)}, \textit{(textIndividual, visIndividual)}, and  \textit{(textGroup, visIndividual)} were approximately the lowest. This was re-affirmed by 

% Experiment 3 also indicates that different visualization combined with text framings do illicit different types of allocation behaviour, when some bias causing unfair allocations is present.
% This means that our effect sizes may have a potential increase if different biases cause higher unfair allocations.
% Our first two experiments indicated that minimal cognitive biases, such as compassion fade, were present when comparing across a proportion of 1:4 victims across two group, unlike as reported prior psychology literature \cite{butts2019helping}.
% However in the third experiment, changing the proportion of victims to a ratio of 1:40 was able to make biases more pronounced, and participants more unfair, across all conditions.
% We still presumes that participants would be more unfair as effects like drop-in-the-bucket would seem to indicate that participants would have chosen a \emph{minority-skewed} allocation strategy, however the \emph{mixed} allocation strategy was still chosen to be in the majority.
% Participants still indicated that that they still wanted to give more to the Zefa group due to more participants, potentially meaning that even if we set the proportion of victims to larger, participants would still would not have chosen the \emph{minority-skewed} allocation strategy.

% In previous experiments had found that fair allocation was the dominant strategy however this was not the case in Experiment 3 where participants commonly donated less than fairly towards Zefa.



% This potentially means biases such as compassion fade may have influence may have been stronger in this study, however, still not as pronounced as stated in prior literature.
% Looking at participant responses, we were did confirm that most participants in the mixed allocation condition did want to donate more to the Zefa condition, meaning that people allocated closely to the fair allocation, even if not exactly fairly.
% While we found that our individual visualization framing did not help mitigate unfairness generally, we did find some evidence in our secondary question that framing visualizations in the presence of a group text framing.
% This is an important consideration as this means that visualization framing is able to mitigate effects from 
% \flag{
% \begin{itemize}
%     \item unfairness was similar for (textGroup, visIndividual), (textIndividual, visIndividual), (textIndvidual, visNone) -- say hwo this compares from exp 2
%     \item also talk about how previous framings contrast to exp 1+2 design
% \end{itemize}
% }
% \flag{While our main research question on the effect of a visualization was inconclusive, we did find some evidence in our secondary question that framing visualizations in a person framing could aid users make fair allocations when a group text is present. 
% Due to multiplicity issues though, we do not conclude this as a strong finding.
% However we think it is still worth emphasizing as other allocation tools presenting a person numerical framing may not always be relevant, for example it may imply resource as being distributed are affecting everyone equally within the group in some cases.}
% \flag{Even if vis is only as good as text, it is a promising approach, since there might be other benefits, not studied in this Experiment.
% Even though it may be the case that visualizations promote similar allocation behaviour as text, the addition visualizations in resource allocation tools may have other benefits unrelated to fair allocations.}
% It is also important to take this finding with respect to prior work, as studies have previously indicated limited findings for visualizations conveying prosociality \cite{morais2021can} within our domain.
% However our results showcase that there is more research within this area as certain anthropological 

==> archives/archive-with-comments-Sep14/08-discussion.tex <==
\section{Discussion and Future Work}

This section discusses our findings, limitations, and research implications.

\subsection{What matters when the goal is promoting fair allocations?}

This work explored the influence of data visualization and information framing for promoting fair resource allocation. We found that allocations seem to be fairer when the information was framed around individuals rather than groups. Our findings also suggest that visualizations are more effective when they are individual-framed and accompanied by textual information. Those findings contribute to advance the understanding of framing in the context of information visualization and shed light on possible research directions. We discuss our results in more detail and their implications in the next paragraphs.

Our experiments are a first attempt to understand the interplay between visualizations, framing, and cognitive biases for the resource allocation problem. Our first experiment contributed to identify strategies used to allocate resources. Interestingly, most participants chose \emph{fair} or \emph{mixed} allocations. Those findings might indicate that our task or tool hindered some cognitive biases and influenced participants to donate more fairly. We should also note that the compassion fade effect seems to be present due to the increase in mixed allocations in the third experiment, but its effect was milder than previous reports \flag{\cite{TODO}}. Contrary to our expectations, other cognitive biases such as the drop-in-the-bucket effect or diversification bias might not have played a major role on the decision-making process since strategies such as \emph{minority-skewed} or \emph{naive} allocations were not common. Our first experiment also brought the first pieces of evidence about the effect of presentation format and information framing for promoting fair allocation, which were confirmed in the next study.

%Initially we presumed that participants would allocate to different strategies as effects like drop-in-the-bucket would seem to indicate that participants would have chosen a \emph{minority-skewed} allocation strategy, however the \emph{mixed} and \emph{fair} allocation strategies were still often in the top-2 majority. During our content analysis in Experiments 1 and 3, participants often indicated that that they wanted to give more to the Zefa program, potentially meaning that even if we set the proportion between the victims of the two programs to be larger, participants would likely still not have chosen the \emph{minority-skewed} allocation strategy.

% Our first experiment tried to find different allocation strategies and amount participants roughly allocated when presented with different framings of our text and visualization design. While we found mostly inconclusive evidence that the presentation format has an effect of fair allocations, we did find a weak evidence for framing. Our procedure may also have led to further confusion. Since we found that participants choose the fair strategy primarily, it also encouraged us to investigate effects based on the proportion of participants who allocate fairly vs unfairly.

The second experiment contributed to solidify the findings from the previous study, using a different metric. Both studies point that combining a data visualization with text using a congruent framing might be as effective as presenting only textual information. On top of that, individual framing seems to cause a higher proportion of fair allocations, independently of the presentation format used. Those findings are promising because it means that adding complementary information through a visualization does not affect the allocations negatively. Therefore, designers could use a visualization with the intent of producing additional benefits to the resource allocation campaign. We discuss more about those implications in \autoref{subsec:what-does-this-mean}. %Finally, it is also important to notice that the proportion of fair allocations in the first two experiments was high for all conditions, meaning that it would be hard to find a small effect.


%In the second experiment, after changes to instruction and measure, we found minimal effects meaning as a large proportion of participants allocated similarly using a fair strategy. This was unexpected as comparing across a proportion of 1:4 victims should have resulted in stronger biases found in prior psychology literature \cite{butts2019helping}.

In the last experiment, we investigated the effect of information framing on resource allocation in more detail, separating the effects by presentation format. Our results suggest that individual framing plays an important role on producing fair allocations, which is in line with the findings from the previous experiments. We could also reinforce the evidence that a \emph{congruent individual framing} (i.e., textIndividual and visIndividual), indeed, seems to be as effective as only using an individual-framed text. Conversely, we could not find evidence that a \emph{congruent group framing} (i.e., textGroup and visGroup) has a similar effect. Regarding incongruent framings, the only effective strategy seemed to be using an individual-framed visualization with a group-framed text. Although those tentative findings are promising and exciting, further studies should be conducted to explore the effect of framing congruence on resource allocation in order to make stronger claims.

% We tried to increase the effect sizes extending the number of participants and potentially inducing stronger biases by changing the proportion of victims to a ratio of 1:40. The latter strategy seemed to work since the proportion of mixed allocations was considerably higher compared to previous studies.

% We also increased the number of participants and changed the proportion of victims to a ratio of 1:40 to potentially induce stronger biases (e.g., compassion fade effect). In doing so, we aimed to investigate the extent to which the previous effects hold in a different scale.

\subsection{Limitation}
\flag{Fanny claims this section}
One of our core limitation of the study was our methods of measurements. 
We decided to give fairness a narrow meaning of donating equally across both in-group and out-group members.
However, people have different opinions and presences so ultimately, many equally correct interpretations of fairness exists.
Furthermore, our metrics of measurements such as the unfairness distance are valid when comparing two charities only.
They will need to be generalized when deciding of an unfairness score for three or more charities.
In this case, a general form of the euclidean distance could be used or a weighted euclidean distance if certain group need to be emphasised or de-emphasised.

Overall, we made simplifying assumptions, namely that the people in the two groups need the donations equally and two charity programs are equally effective. However, it is evident that people don't have equal needs and charity programs differ vastly in their effectiveness \cite{dragicevic2022information}.
To handle cases like these, we will need tools that are much more elaborate than our simple allocation tool, which we should clearly present as a tool for doing experiments and understand how people make allocation decisions and the trade-offs between design choices, not as something that is meant to be deployed in real settings.

To handle cases like these, a more robust and complex tool must be built to evaluate how people make allocation decisions and which trade-offs in the design choices are the most impactful to those decisions.
Our simple tool was made for experimental purposes only and is not readily available to be deployed in the far more complex setting of the real-world.

\subsection{What does this mean?}
\label{subsec:what-does-this-mean}


\subsubsection{Visualization Design}
\fix{integrate interaction in there -- Fanny can work on this, ot Luiz+Fanny convene in the afternoon to work on these two sections}
Unlike prior research, we attempt to merge theories in framing, cognitive biases concerning affect, and visualization to explore interactive tool designs which help mitigate unfairness from biases.
While our results are not able to confidently prescribe new visualization design for reducing unfairness due to inconclusive or tentative findings, we do find that individual visualization framing is able to be as good presenting individual text and actually beneficial when there is group text framing, in terms of fairness.
Our finding add nuance to previous studies which found little influence of visualizations in inducing prosocial behaviors \cite{morais2021can}.
This is an important finding as there are real world constraints to consider when integrating both text and visualization. It may not always be possible to present text in a certain type of framing, i.e. if the visualization was to be integrated alongside a news articles where allocations are usually reported in a group framing. Presenting an alternate framing for text may confuse the reader, however, the integration of a certain visualization may capture their attention.
In this case, it is important to know which framings are the most useful in communicating information.

Our allocation visualization design can also be integrated in many contexts, as such there are also many more dimensions from which we can alter the design to guide fairness. 
For example, our marks for representing group populations anthroprographics \cite{morais2020showing} can be used to represent the diverse population samples instead of traditionally male glyph iconography. Other resource commonly used for allocation such as time could also be represented instead of the coins visualized.

\flag{
Visualizations don't necessarily have to promote fairness either, rather, as long as unfairness is not induced, they can provide other benefits. Integrating such interactive visualization can help build interactive articles which help draw engagement \cite{hohman2020communicating}, and can even promote self-reflection \cite{chi1989self}. Interactive visualization also be further be leveraged to allow for dynamic content engagement \cite{shneiderman2003eyes}. 
}

\flag{Playfulness of visualization -- more engaging, enticing, grab attention.}


\subsection{Allocation Tools}
In general, we use our study as an exploratory guide on how visualization framing may be utilized and studied for designing resource allocation tools.
Such tools exist with limited capacity to compare the effectiveness of resources allocated across charities.
Our study used only a slider as a simple method of input but there are many others such as hand gestures on touch or 3D displays.
Such methods and interactive visualizations may add additional benefit for the user such as an increase in engagement.

\textbf{Automation.} Modern web scraping capabilities and the prediction of donation effectiveness could allow for the tools similar to the one we have shown to generalize across many news articles.
Large databases for grant allocation already exist such as the official site for USA government spending (https://www.usaspending.gov).
As such, integration of allocation tools with data in the wild is extremely plausible and could be impactful for a significantly wider audience.
There can also be more static content displayed on the tool's interface, given futher extracted information, such as representing the probabilistic aspect for charitable donation, resources already allocated to the existing groups, and further time constraints.

% While our tool contains integrated text, this can also be incorporated in-situ visualizations with text processing.
\textbf{Going further.} There has been recent work in improving automated and heuristics-based assistance for the allocation of resources for humanitarian aid \cite{aiken2022machine, anparasan2019resource, callaway2022rational}.
However if regular visualizations are used for such showcasing allocations, there are may problems with framing the visualizations and biasing observers to heavily distrust or rely on the results of an automated system.
Our research showcases tentatively that the information and results communicated for an allocation may make people think a donation was fair or unfair, regardless of the actual effectiveness. 
The utility of resource allocation tools is not simply for donors themselves but could also be used for visualizing an automated amount given out by some system such as one integrating a machine learning model.
Such tools provide ways to alleviate potential harms in an algorithmically-infused societies \cite{wagner2021measuring}.




% text and visualization design, we tested to see which allocation strategies participants commonly used. 

% text information or visualizations and changes in framing tobto


% we find mostly inconclusive evidence that the addition of visualizations and changes in framing, specifically a person framing compared to a group framing, has an effect on allowing people to allocate resources more fairly.
% However in our third experiment we have tentative findings that visualizations with an individual framing could allow for allocations which are just as fair 

% While we did find some evidence that framing visualizations in an individual framing could aid people in making fair allocations when in the presence of a group numerical framing, due to multiplicity issues we conclude this as a tentative finding.


% However in the third experiment, changing the proportion of victims to a ratio of 1:40 was able to make biases more pronounced, and participants more unfair, across all conditions.

% Experiment 3 also indicates that different visualization combined with text framings do illicit different types of allocation behaviour, when some bias causing unfair allocations is present.
% This means that our effect sizes may have a potential increase if different biases cause higher unfair allocations.

% Something we want to take about is hte effect of insturction

% Having \emph{inidvidualVis} promote fairer allocation when it was presented with an incongrutent text 

% About 2a) above, maybe we can mention research that is using AI to try to find who needs money the most. I think Arnav sent something about it.
% But there are other, simpler ways that are currently used by organizations like Give Directly. I can try to find the ref if needed.

% Among the limitations, we should probably emphasize that our study focused on a very simplified decision task:
% People are asked to allocate between two charity programs, but the number of options might be dozens or hundreds
% There are lots of simplifying assumptions, including that a) the people in the two groups need the donations equally and that b) the two charity programs are equally effective. It’s well known that a) people dont’ have equal needs, if only because there are vast inequalities basically anywhere on Earth. Also, b) charity programs differ vastly in their effectiveness (you can cite my little essay on EA which is now on Arxiv https://arxiv.org/abs/2209.00836). To handle cases like these, we will need tools that are much more elaborate than our simple allocation tool, which we should clearly present as a tool for doing experiments and understand how people make allocation decisions and the trade-offs between design choices, not as something that is meant to be deployed in real settings.
% In the real world, there are huge uncertainties (e.g., about how effective a charity program will actually be). We don’t consider this in this paper.


%     \item Limitations of our work: we have oversimplified scenarios. In real life, there's many more factors to the scenarios. The same resources are not equivalent across different individuals and can impact them differently. The needs are not exactly the same. Should this information be embedded visually, and how?

% • visualization may be a tool worth investigating further for
% these types of tools. Our work shows that design decisions
% can impact. There are many more aspects in the visual design
% that can play a role: different icons to represent the diverse
% population (see anthropomorphism), other layouts, resources
% that are not as tangible as money (e.g. time), also impact of
% resources (e.g. 1 coin may impact one 10times more than an
% another one)... Need for much more research to investigate the
% effects of techniques and parameters
% • should we have interaction? we’re exploring the ”what-if”
% scenarios in an interactive manner. What are the implications
% of that? Can it be made richer?
% • Limitations of our work: we have oversimplified scenarios.
% In real life, there’s many more factors to the scenarios. The
% same resources are not equivalent across different individuals
% and can impact them differently. The needs are not exactly
% the same. Should this information be embedded visually, and
% how?
% • Should the design be left to the designer? Can computational
% tools help here? Cite ML work on the topic.
% • Where should these tools be integrated? How to feed the tools
% with the actual data?


==> archives/archive-without-a-date/macros.tex <==
%\usepackage{fixme}
%\fxsetup{status=draft, layout=inline, theme=color}
% fixme package provides note, warning, error, fatal for each registered author
%\FXRegisterAuthor{av}{aam}{arnav}
%\FXRegisterAuthor{fc}{aam}{fanny}

% usage
%\avnote{I like the fixme package!}
%\avwarning{I like the fixme package!}
%\averror{I like the fixme package!}

% \avnote{This is a text comment}




\usepackage{colortbl}                  
\usepackage{framed}
%\usepackage{enumitem}
\usepackage[inline,shortlabels]{enumitem}

% Styling macro for in-text quotations of text from corpus papers
\newcommand{\myquote}[1]{\textit{#1}}

% Fix missing \paperheight warning, using Overleaf default size
\setlength{\paperheight}{11in}

% --- Author in-text comment macros. Comment out these lines in final version and check for errors to make sure all our comments are removed.
\newcommand{\arnav}[1]{\textcolor{magenta}{[AV: #1]}}
\newcommand{\fanny}[1]{\textcolor{violet}{[FC: #1]}}
\newcommand{\pierre}[1]{\textcolor{teal}{[PD: #1]}}
\newcommand{\luiz}[1]{\textcolor{orange}{[LM: #1]}}
\newcommand{\emphb}[1]{\textbf{\emph{#1}}}
\newcommand{\fix}[1]{\textcolor{red}{#1}}

%% Non-draft
%\newcommand{\arnav}[1]{\textcolor{magenta}{}}
%\newcommand{\fanny}[1]{\textcolor{violet}{}}
%\newcommand{\pierre}[1]{\textcolor{teal}{}
%\newcommand{\luiz}[1]{\textcolor{orange}{}


\newcommand{\flag}[1]{\textcolor{red}{#1}}
\newcommand{\reuse}[1]{\textcolor{black}{#1}}
\newcommand{\reused}[1]{\textcolor{green}{#1}}
% ---



\usepackage{float}
\usepackage{scrextend}

% --- File outline and PDF bookmark outline setup
% Give PDF files a nice bookmark outline
\usepackage[numbered, depth=4]{bookmark}

% Make \paragraph header not display in text, so can use it for file outline and TOC/PDF bookmarks without showing in text. Mainly used in taxonomy section for tasks definition sections, which are made with macros and custom formatting.
\usepackage{titlesec}
\makeatletter
\titleformat{\paragraph}[runin]{}{}{0pt}{\@gobble}
\makeatother
\titlespacing{\paragraph}{\parindent}{0pt}{0pt}
% ---


% ----- Phase (before renaming to Category) and Task Macros -------------------------------------------
% phase
\usepackage{xspace}
\newcommand{\phase}{Category\xspace}
\newcommand{\phases}{Categories\xspace}

% inline phase number and description. Example: Phase 1 (...)
% arguments: phase #, description
\newcommand{\phaseInline}[2]{\phase #1 (#2)}

% task name. Example: P1-T1
% arguments: phase #, task #
%\newcommand{\taskName}[2]{P#1-T#2}
%\newcommand{\taskName}[2]{#1$\rightarrow$#2}

%\newcommand{\taskName}[2]{#1.#2}

% inline task name and description. Example: P1-T1 (description)
% arguments: phase #, task #, description
\newcommand{\taskInline}[3]{\taskName{#1}{#2} (#3)}

% --- Delete items above this line once they are no longer used, which is when we've switched whole paper over to the new category:task scheme.

% -- Macros for Category and task display styles

% Reference task in the text
% arguments: category name, task short name
\newcommand{\taskName}[2]{#1\,$\rhd$\,#2}

% Regular mini-section for defining an inspection task
% arguments: category name, task short name, task description
\newcommand{\taskShortTitle}[3]{
\vspace*{1em}
\begin{leftbar}
% original version %\noindent{\small \textbf{\taskName{#1}{#2}}:} \textit{#3}
% revised version
\noindent{\small \textbf{\taskName{#1}{#2}}:} #3
\end{leftbar}
}

% First occurrence of mini-section \taskShortTitle, with explicit naming scheme.
% Only used for the first task. Use \taskShortTitle everywhere else.
% arguments: category name, task short name, task description
\newcommand{\taskTitle}[3]{
\vspace*{1em}
\begin{leftbar}
\noindent {\small \textbf{\taskName{#1}{#2} (Category: #1, Task: #2)}:} \textit{#3}
\end{leftbar}
}

% ----------------------------------------------------------------


% --- Wrap figure macro
\usepackage{wrapfig}

% Thank you Silvia
\newcommand{\wf}[6]{%
  \vspace*{-0.5\intextsep}
  \hspace*{-0.5\columnsep}
  \begin{wrapfigure}[#1]{#2}{#3}%
  \centering%
  \includegraphics[#4]{#5}
  #6%
\end{wrapfigure}}
% ---



% Macros for change highlighting

% Package for strike-through of text
\usepackage[normalem]{ulem}

\definecolor{darkgreen}{rgb}{0, 0.5, 0}
\definecolor{differentblue}{rgb}{0, 0.5, 0.8}
\newcommand{\todo}[1]{\textcolor{red}{#1}}


%%%%%%%%%%%%%%%%%%%%%% MACROS FOR ROUND 2

\newcommand{\changedcgf}[2]{#1}
\newcommand{\changedsimplecgf}[1]{#1}
\newcommand{\removedcgf}[1]{}
\newcommand{\addedcgf}[1]{#1}

%\newcommand{\changedcgf}[2]{%
   %#1: new text (green)
   %#2: old text (gray and struck-out)
%    \textcolor{darkgreen}{#1}%
%    \textcolor{gray}{\xspace\sout{#2}\xspace}%
%}
%\newcommand{\changedsimplecgf}[1]{\textcolor{darkgreen}{#1}}
%\newcommand{\removedcgf}[1]{\textcolor{gray}{\sout{#1}}}
%\newcommand{\addedcgf}[1]{\textcolor{differentblue}{#1}}



%%%%%%%%%%%%%%%%%%%%%% MACROS FOR REVISED CAMERA-READY (Not coloured)

\newcommand{\changed}[2]{#1}
\newcommand{\changedsimple}[1]{#1}
\newcommand{\removed}[1]{}
\newcommand{\added}[1]{#1}


%%%%% NOT USED?
\newenvironment{changedtext}[1]
    {\color{darkgreen}
    #1
    }
    {\color{black}
    }
\newenvironment{addedtext}[1]
{\color{blue}
#1
}
{\color{black}
}



%%%%%%%%%%%%%%%%%% LEFT BAR FOR DEFINITIONS

\usepackage{framed}
\usepackage{xcolor}
\newlength{\leftbarwidth}
\setlength{\leftbarwidth}{1pt}
\newlength{\leftbarsep}
\setlength{\leftbarsep}{8pt}
\newcommand*{\leftbarcolorcmd}{\color{leftbarcolor}}% as a command to be more flexible
\colorlet{leftbarcolor}{black}
\renewenvironment{leftbar}{%
    \begin{samepage}
    \vspace{2mm}
    \def\FrameCommand{{\leftbarcolorcmd{\vrule width \leftbarwidth\relax\hspace {\leftbarsep}}}}%
    \MakeFramed {\advance \hsize -\width \FrameRestore }%
}{%
    \endMakeFramed
    \end{samepage}
}

% Final version - redefine macros to hide removed text, etc.


==> archives/archive-without-a-date/main_old.tex <==

%%
%% End of file `sample-authordraft.tex'.

% % $Id: template.tex 11 2007-04-03 22:25:53Z jpeltier $

% % \documentclass[sigconf]{acmart}
% \documentclass{vgtc}                          % final (conference style)
% %\documentclass[review]{vgtc}                 % review
% %\documentclass[widereview]{vgtc}             % wide-spaced review
% %\documentclass[preprint]{vgtc}               % preprint
% %\documentclass[electronic]{vgtc}             % electronic version

% %% Uncomment one of the lines above depending on where your paper is
% %% in the conference process. ``review'' and ``widereview'' are for review
% %% submission, ``preprint'' is for pre-publication, and the final version
% %% doesn't use a specific qualifier. Further, ``electronic'' includes
% %% hyperreferences for more convenient online viewing.

% %% Please use one of the ``review'' options in combination with the
% %% assigned online id (see below) ONLY if your paper uses a double blind
% %% review process. Some conferences, like IEEE Vis and InfoVis, have NOT
% %% in the past.

% %% Figures should be in CMYK or Grey scale format, otherwise, colour 
% %% shifting may occur during the printing process.

% %% These few lines make a distinction between latex and pdflatex calls and they
% %% bring in essential packages for graphics and font handling.
% %% Note that due to the \DeclareGraphicsExtensions{} call it is no longer necessary
% %% to provide the the path and extension of a graphics file:
% %% \includegraphics{diamondrule} is completely sufficient.
% %%
% \ifpdf%                                % if we use pdflatex
%   \pdfoutput=1\relax                   % create PDFs from pdfLaTeX
%   \pdfcompresslevel=9                  % PDF Compression
%   \pdfoptionpdfminorversion=7          % create PDF 1.7
%   \ExecuteOptions{pdftex}
%   \usepackage{graphicx}                % allow us to embed graphics files
%   \DeclareGraphicsExtensions{.pdf,.png,.jpg,.jpeg} % for pdflatex we expect .pdf, .png, or .jpg files
% \else%                                 % else we use pure latex
%   \ExecuteOptions{dvips}
%   \usepackage{graphicx}                % allow us to embed graphics files
%   \DeclareGraphicsExtensions{.eps}     % for pure latex we expect eps files
% \fi%


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%% PACKAGES %%%%%%%%%%%%%%%%%%%%%%
% \usepackage{hyperref}

% \hypersetup{
%     colorlinks=true,
%     linkcolor=blue,
%     filecolor=magenta,      
%     urlcolor=cyan,
%     pdftitle={Overleaf Example},
%     pdfpagemode=FullScreen,
%     }

% \urlstyle{same}


% \input{macros}

% %% it is recomended to use ``\autoref{sec:bla}'' instead of ``Fig.~\ref{sec:bla}''
% \graphicspath{{figures/}{pictures/}{images/}{./}} % where to search for the images

% \usepackage{microtype}                 % use micro-typography (slightly more compact, better to read)
% \PassOptionsToPackage{warn}{textcomp}  % to address font issues with \textrightarrow
% \usepackage{textcomp}                  % use better special symbols
% \usepackage{mathptmx}                  % use matching math font
% \usepackage{times}                     % we use Times as the main font
% \renewcommand*\ttdefault{txtt}         % a nicer typewriter font
% \usepackage{cite}                      % needed to automatically sort the references
% \usepackage{tabu}                      % only used for the table example
% \usepackage{booktabs}                  % only used for the table example
% %% We encourage the use of mathptmx for consistent usage of times font
% %% throughout the proceedings. However, if you encounter conflicts
% %% with other math-related packages, you may want to disable it.
% \usepackage{graphicx}
% \usepackage{subcaption}
% \usepackage{mwe}



% %% If you are submitting a paper to a conference for review with a double
% %% blind reviewing process, please replace the value ``0'' below with your
% %% OnlineIDF. Otherwise, you may safely leave it at ``0''.
% \onlineid{0}

% %% declare the category of your paper, only shown in review mode
% \vgtccategory{Research}

% %% allow for this line if you want the electronic option to work properly
% % \vgtcinsertpkg

% %% In preprint mode you may define your own headline.
% %\preprinttext{To appear in an IEEE VGTC sponsored conference.}

% %% Paper title.

% \title{Reasoning Beyond the Numbers: \\ 
% Can Framing Influence Effective Resource Allocations?}

% %% This is how authors are specified in the conference style

% %% Author and Affiliation (single author).
% %%\author{Roy G. Biv\thanks{e-mail: roy.g.biv@aol.com}}
% %%\affiliation{\scriptsize Allied Widgets Research}

% %% Author and Affiliation (multiple authors with single affiliations).
% %%\author{Roy G. Biv\thanks{e-mail: roy.g.biv@aol.com} %
% %%\and Ed Grimley\thanks{e-mail:ed.grimley@aol.com} %
% %%\and Martha Stewart\thanks{e-mail:martha.stewart@marthastewart.com}}
% %%\affiliation{\scriptsize Martha Stewart Enterprises \\ Microsoft Research}

% %% Author and Affiliation (multiple authors with multiple affiliations)
% \author{Arnav Verma\thanks{e-mail:arnav@dgp.toronto.edu}\\ %
%         \scriptsize University of Toronto %
% \and Luiz Morais\thanks{e-mail:luiz.morais@inria.fr}\\ %
%      \scriptsize INRIA %
% \and Pierre Dragicevic\thanks{e-mail:pierre.dragicevic@inria.fr}\\ %
%      \parbox{1.4in}{\scriptsize \centering INRIA}
% \and Fanny Chevalier\thanks{e-mail:fanny@dgp.toronto.edu}\\ %
%      \parbox{1.4in}{\scriptsize \centering University of Toronto}}

% %% A teaser figure can be included as follows, but is not recommended since
% %% the space is now taken up by a full width abstract.
% %\teaser{
% %  \includegraphics[width=1.5in]{sample.eps}
% %  \caption{Lookit! Lookit!}
% %}

% %% Abstract section.
% \abstract{
% \todo{XXXXXX}
% } % end of abstract

% %% ACM Computing Classification System (CCS). 
% %% See <http://www.acm.org/class/1998/> for details.
% %% The ``\CCScat'' command takses four arguments.

% \CCScatlist{ 
%   \CCScat{K.6.1}{Management of Computing and Information Systems}%
% {Project and People Management}{Life Cycle};
%   \CCScat{K.7.m}{The Computing Profession}{Miscellaneous}{Ethics}
% }

% %% Copyright space is enabled by default as required by guidelines.
% %% It is disabled by the 'review' option or via the following command:
% % \nocopyrightspace

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%% START OF THE PAPER %%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{document}

% %% The ``\maketitle'' command must be the first command after the
% %% ``\begin{document}'' command. It prepares and prints the title block.

% %% the only exception to this rule is the \firstsection command

% \input{01-introduction}
% \input{02-background}
% \input{2.5-vis-design}
% \input{03-study1}
% \input{04-study2}
% \input{05-study3}
% \input{06-discussion}
% \input{07-conclusion}


% %% if specified like this the section will be committed in review mode
% \acknowledgments{
% The authors wish to thank A, B, C. This work was supported in part by
% a grant from XYZ.
% }

% %\bibliographystyle{abbrv}
% \bibliographystyle{abbrv-doi}
% %\bibliographystyle{abbrv-doi-narrow}
% %\bibliographystyle{abbrv-doi-hyperref}
% %\bibliographystyle{abbrv-doi-hyperref-narrow}

% \bibliography{bibliography}
% \end{document}


==> archives/temp.tex <==
% studies that investigated humanitarian decision-making processes in empirical and descriptive ways.

Making a decision, where humanitarian causes are concerned, is often reliant on many external factors which depend on the information exposed to the decision-maker. Individuals will often conduct information-seeking or avoidance based on prior biases \cite{sharot2020people}. Information seeking may be minimal for institutional decision-makers, such as operational agencies, as well. Reports indicate that assessments for humanitarian need may often depend as much on prediction as they do on observed fact \cite{darcy2003according}, leaving room for further biases from individuals to be introduced. 
Thus, even when the recorded information for different events is similar, the final allocation may relies on the individual.

% This means for many humanitarian decision-makers, the decision making process can be prone to biases such as the framing effect \cite{gosling2020interplay}. 

% ChatGPT
% When making decisions involving humanitarian issues, many external factors that affect the decision-making process can be influenced by the information available to the decision-maker. These individuals may engage in information-seeking or avoidance behaviors based on their existing biases \cite{sharot2020people}. Even institutional decision-makers, such as operational agencies, may not always seek out all relevant information. As a result, assessments of humanitarian needs may rely on predictions rather than observed facts \cite{darcy2003according}, which can introduce further bias into the decision-making process. This can lead to the influence of biases such as the framing effect \cite{gosling2020interplay} on the decision-making process

==> figures/exp-1-bar.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.475\textwidth}
        \centering
        \includegraphics[width=\textwidth]{pictures/exp_1_analysis/text-cause-bar.png}
        \caption[]%
        {{\small Per-cause framing and text presentation format}}    
        \label{fig:text-cause-bar}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.475\textwidth}  
        \centering 
        \includegraphics[width=\textwidth]{pictures/exp_1_analysis/text-person-bar.png}
        \caption[]%
        {{\small Per-person framing and text presentation format}}
        \label{fig:text-person-bar}
    \end{subfigure}
    \vskip\baselineskip
    \begin{subfigure}[b]{0.475\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{pictures/exp_1_analysis/vis-cause-bar.png}
        \caption[]%
        {{\small Per-cause framing and visualization presentation format}}
        \label{fig:vis-cause-bar}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.475\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{pictures/exp_1_analysis/vis-person-bar.png}
        \caption[]%
        {{\small Per-person framing and visualization presentation format}}    
        \label{fig:vis-person-bar}
    \end{subfigure}
    \caption[]
    {Donation amount towards program Zefa (12 children). } 
    \label{fig:exp_1_bar}
\end{figure*}

==> figures/exp-1-contrast.tex <==
\begin{figure}
    \centering
    \begin{subfigure}[b]{0.95\linewidth}
        \centering
        \includegraphics[width=\linewidth]{pictures/exp_1_analysis/dom-framing.png}
        \caption[]%
        {{\small}}    
        \label{fig:exp_1_dom_framing}
    \end{subfigure}
    \vskip\baselineskip
    \begin{subfigure}[b]{0.95\linewidth}  
        \centering 
        \includegraphics[width=\linewidth]{pictures/exp_1_analysis/dom-pres.png}
        \caption[]%
        {{\small }}
        \label{fig:exp_1_dom_pres}
    \end{subfigure}
    \vskip\baselineskip
    \begin{subfigure}[b]{0.95\linewidth}   
        \centering 
        \includegraphics[width=\linewidth]{pictures/exp_1_analysis/dom-pres.png}
        \caption[]%
        {{\small}}
        \label{fig:exp_1_dom_interact}
    \end{subfigure}
    \caption[]
    {Inferential statistics for difference of means and interaction between our variables} 
    \label{fig:exp_1_contrasts}
\end{figure}

==> figures/exp-1-design.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.475\textwidth}
        \centering
        \includegraphics[width=\textwidth]{pictures/exp_1_figs/per_cause_novis_1.png}
        \caption[]%
        {{\small Per-cause framing and text presentation format}}    
        \label{fig:per_cause_novis_1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.475\textwidth}  
        \centering 
        \includegraphics[width=\textwidth]{pictures/exp_1_figs/per_person_novis_1.png}
        \caption[]%
        {{\small Per-person framing and text presentation format}}
        \label{fig:per_person_novis_1}
    \end{subfigure}
    \vskip\baselineskip
    \begin{subfigure}[b]{0.475\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{pictures/exp_1_figs/per_cause_vis_1.png}
        \caption[]%
        {{\small Per-cause framing and visualization presentation format}}
        \label{fig:per_cause_vis_1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.475\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{pictures/exp_1_figs/per_person_vis_1.png}
        \caption[]%
        {{\small Per-person framing and visualization presentation format}}    
        \label{fig:per_person_vis_1}
    \end{subfigure}
    \caption[]
    {Allocation task design for experiments 1 and 2. } 
    \label{fig:exp_1_design}
\end{figure*}

==> figures/exp-1-donations.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{pictures/exp_1_analysis/mean-err.png}
        \caption[]%
        {{\small Mean response for each of the four conditions (95\% bootstrap CIs)}}    
        \label{fig:exp_1_donations_mean_ci}
    \end{subfigure}
    \begin{subfigure}[b]{0.5\textwidth}  
        \centering 
        \includegraphics[width=\textwidth]{pictures/exp_1_analysis/stacked-bar.png}
        \caption[]%
        {{\small Proportions of responses per category}}
        \label{fig:exp_1_donations_cat_prop}
    \end{subfigure}
    \hfill
    \vskip\baselineskip
    \caption[]
    {Visual comparison of the amount Donated to program Zefa, across each condition.} 
    \label{fig:exp_1_donations}
\end{figure*}

==> figures/exp-3-contrast.tex <==
\begin{figure}
    \centering
    \begin{subfigure}[b]{0.95\linewidth}
        \centering
        \includegraphics[width=\linewidth]{pictures/exp_3/framing_influence.png}
        \caption[]%
        {{\small}}    
        \label{fig:exp_3_framing_influence}
    \end{subfigure}
    \vskip\baselineskip
    \begin{subfigure}[b]{0.95\linewidth}  
        \centering 
        \includegraphics[width=\linewidth]{pictures/exp_3/vis_framing.png}
        \caption[]%
        {{\small }}
        \label{fig:exp_3_vis_framing}
    \end{subfigure}
    \vskip\baselineskip
    \begin{subfigure}[b]{0.95\linewidth}   
        \centering 
        \includegraphics[width=\linewidth]{pictures/exp_3/intreaction.png}
        \caption[]%
        {{\small}}
        \label{fig:exp_3_intreaction}
    \end{subfigure}
    \caption[]
    {Inferential statistics for difference of means and interaction between our variables} 
    \label{fig:exp_3_contrasts}
\end{figure}

==> figures/exp-3-design.tex <==
\begin{figure*}
    \centering
    \hfill
    \begin{subfigure}[b]{0.33\textwidth}  
        \centering
        \caption[]%
        {{\small No Text and No Visualization (Omitted) }}
        \label{fig:no_txt_vis_3}
    \end{subfigure}
    \begin{subfigure}[b]{0.33\textwidth}
        \centering
        \includegraphics[width=\textwidth]{pictures/exp_3/figs/group_text_no_vis.png}
        \caption[]%
        {{\small Group Text and No Visualization}}    
        \label{fig:group_text_no_vis_3}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.33\textwidth}  
        \centering 
        \includegraphics[width=\textwidth]{pictures/exp_3/figs/person_text_no_vis.png}
        \caption[]%
        {{\small Person Text and No Visualization}}
        \label{fig:no_text_group_vis_3}
    \end{subfigure}
    \vskip\baselineskip
     
    \begin{subfigure}[b]{0.33\textwidth}  
        \centering 
        \includegraphics[width=\textwidth]{pictures/exp_3/figs/no_text_group_vis.png}
        \caption[]%
        {{\small No Text and Group Visualization}}
        \label{fig:person_text_no_vis_3}
    \end{subfigure}
    \begin{subfigure}[b]{0.33\textwidth}  
        \centering 
        \includegraphics[width=\textwidth]{pictures/exp_3/figs/group_text_group_vis.png}
        \caption[]%
        {{\small Group Text and Group Visualization }}
        \label{fig:group_text_group_vis_3}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.33\textwidth}
        \centering
        \includegraphics[width=\textwidth]{pictures/exp_3/figs/person_text_group_vis.png}
        \caption[]%
        {{\small Person Text and Group Visualization}}    
        \label{fig:person_text_group_vis_3}
    \end{subfigure}
    \vskip\baselineskip
    
    \begin{subfigure}[b]{0.33\textwidth}  
        \centering 
        \includegraphics[width=\textwidth]{pictures/exp_3/figs/no_text_person_vis.png}
        \caption[]%
        {{\small No Text and Person Visualization }}
        \label{fig:no_text_person_vis_3}
    \end{subfigure}
    \begin{subfigure}[b]{0.33\textwidth}
        \centering
        \includegraphics[width=\textwidth]{pictures/exp_3/figs/group_text_person_vis.png}
        \caption[]%
        {{\small Group Text and Person Visualization  }}    
        \label{fig:group_text_person_vis_3}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.33\textwidth}  
        \centering 
        \includegraphics[width=\textwidth]{pictures/exp_3/figs/person_text_person_vis.png}
        \caption[]%
        {{\small Person Text and Person Visualization}}
        \label{fig:person_text_person_vis_3}
    \end{subfigure}
    \caption[]
    {Allocation task design for experiments 3. } 
    \label{fig:exp_3_design}
\end{figure*}

==> figures/exp-3-donations.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{pictures/exp_3/mean_err.png}
        \caption[]%
        {{\small Mean response for each of the four conditions (95\% bootstrap CIs)}}    
        \label{fig:exp_3_donations_mean_ci}
    \end{subfigure}
    \begin{subfigure}[b]{0.5\textwidth}  
        \centering 
        \includegraphics[width=\textwidth]{pictures/exp_3/stacked_bar.png}
        \caption[]%
        {{\small Proportions of responses per category}}
        \label{fig:exp_3_donations_cat_prop}
    \end{subfigure}
    \hfill
    \vskip\baselineskip
    \caption[]
    {Visual comparison of the amount Donated to program Zefa, across each condition.} 
    \label{fig:exp_3_donations}
\end{figure*}
